Efficient Inverse Multiagent Learning

In this paper, we study inverse game theory (resp. inverse multiagent learning) in which the goal is to find parameters of a game's payoff functions for which the expected (resp. sampled) behavior is an equilibrium. We formulate these problems as generative-adversarial (i.e., min-max) optimization problems, for which we develop polynomial-time algorithms to solve, the former of which relies on an exact first-order oracle, and the latter, a stochastic one. We extend our approach to solve inverse multiagent simulacral learning in polynomial time and number of samples. In these problems, we seek a simulacrum, meaning parameters and an associated equilibrium that replicate the given observations in expectation. We find that our approach outperforms the widely-used ARIMA method in predicting prices in Spanish electricity markets based on time-series data.

==> Cournot_and_Bertrand.tex <==
\subsubsection{Cournot Competition and Bertrand Competition}

A \mydef{Cournot competition model} $\calC \doteq (\numfirms, \mcost, \pricefunc)$ consists of $n$ firms that produce a homogeneous product, and each firm chooses a quantity level of production that maximizes its profits. The set of \mydef{Cournot Equilibrium} of a Cournot competition model is equal to the set of Nash Equilibrium of a one-shot general-sum game, \mydef{Cournot game} (see more details in \Cref{sec_app:markets}). 

A \mydef{Bertrand competition model} $\calB \doteq (\numfirms, \mcost, \demandfunc)$ is also a competition model that consists of $n$ firms producing a homogeneous product, but this time, each firm set prices to maximize its profits. Similarly, we can compute the \mydef{Bertrand equilibrium} of the model by computing the NE of the one-shot general-sum game, \mydef{Bertrand game} (see more details in \Cref{sec_app:markets}). 

In experiments, we generated 500 Cournot competition models and 500 Bertrand competition models and attempted to retrieve their true parameter, i.e., marginal costs, given equilibrium productions/equilibrium prices respectively. \Cref{table:cournot+bertrand_results} shows that our algorithm can effectively recover the true parameters in Cournot games and minimize the exploitability of the observed equilibrium evaluated under the computed parameters. In the Bertrand games, though we could only recover $78\%$ true parameters, the average exploitability of the observed equilibrium evaluated under the computed inverse Nash equilibrium is mostly minimized. 




==> algos/eda.tex <==
%%% EDA

% \begin{algorithm}[t!]
% \caption{Extragradient descent ascent (EDA)}
% \textbf{Inputs:} $\numplayers, \util, \actions, \learnrate,  \numiters, \strat[][][0], \otherstrat[][][0]$\\
% \textbf{Outputs:} $(\strat[][][\iter], \otherstrat[][][\iter])_{t = 0}^\numiters$
% \label{alg:egda_cumul_regret}
% \begin{algorithmic}[1]
% \For{$\iter = 0, \hdots, \numiters - 1$}
    
%     \State  $\strat[][][\iter + \nicefrac{1}{2}] = \project[\actions] \left[\strat[][][\iter] - \learnrate[ ] \grad[{\strat}] \cumulregret(\strat[][][\iter], \otherstrat[][][\iter]) \right]$
    
%     \State  $\otherstrat[][][\iter + \nicefrac{1}{2}]  = \project[\actions] \left[ \otherstrat[][][\iter] + \learnrate[ ]\grad[{\otherstrat}] \cumulregret(\strat[][][\iter], \otherstrat[][][\iter]) \right]$
    
%     \State $\strat[][][\iter+1] = \project[\actions] \left[\strat[][][\iter ] - \learnrate[ ] \grad[{\strat}] \cumulregret(\strat[][][\iter + \nicefrac{1}{2}], \otherstrat[][][\iter + \nicefrac{1}{2}]) \right]$
    
%     \State $\otherstrat[][][\iter + 1]  = \project[\actions] \left[ \otherstrat[][][\iter] + \learnrate[ ]\grad[{\otherstrat}] \cumulregret(\strat[][][\iter + \nicefrac{1}{2}], \otherstrat[][][\iter + \nicefrac{1}{2}]) \right]$

% \EndFor
% \State \Return $(\strat[][][\iter], \otherstrat[][][\iter])_{t = 0}^\numiters$
% \end{algorithmic}
% \end{algorithm}


==> arrow_debreu.tex <==
\section{Computing Competitive Equilibria in Arrow-Debreu Markets}
\label{sec:arrow_debreu}

\deni{Explain why do you think this was hard.}

A \mydef{Fisher market} $(\numbuyers, \numgoods, \valuation, \budget)$, $(\valuation, \budget)$ when clear from context, consists of $\numbuyers$ buyers and $\numgoods$ divisible goods with unit supply.
Each buyer $\buyer \in \buyers$ has a budget $\budget[\buyer] \in \mathbb{R}_{+}$ and a utility function $\valuation[\buyer]: \consumptions[\buyer] \to \mathbb{R}_+$, where $\consumptions[\buyer] \subseteq \mathbb{R}^{\numgoods}_+$ is buyer $\buyer$'s consumption space \cite{brainard2000compute}.
We denote
%%% SPACE
%the set of 
joint consumptions by $\consumptions = \bigtimes_{\buyer \in \buyers} \consumptions[\buyer]$.

A \mydef{Fisher market competitive equilibrium (FMCE)} is a tuple comprising allocations $\allocation \in \consumptions$ and prices $\price \in \simplex[\numgoods]$ s.t.\ 1.~all buyers $\buyer \in \buyers$ maximize utility constrained by their budget: $\allocation[\buyer]^* \in \argmax_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price \leq \budget[\buyer]} \valuation[\buyer](\allocation[\buyer])$, 2.~the markets clear, meaning the allocation is feasible and Walras' law holds, i.e., $ \sum_{\buyer \in \buyers} \allocation[\buyer]^*  \leq \ones[\numgoods]$ and $\price^* \cdot \left( \sum_{\buyer \in \buyers} \allocation[\buyer]^*  - \ones[\numgoods] \right) = 0$. 
% \amy{i thought we decided that the first condition was feasbility, and the second, Walras' law.}

% Without loss of generality, we assume that there is one divisible unit of each good in the market \cite{AGT-book}.

% The seller's utility $\valuation[0]: \mathbb{R}_{+}^{\numgoods} \to \mathbb{R}_+$ is given by $\valuation[0](\allocation[0]) = \allocation[0][\numbuyers+1]$, while the 

%\amy{i am not sure where this next paragraph is coming from. there is no reference? and there is no proof. is this something we have already shown, b/c i don't recall us talking about FMCE as Nash eqa, but only as SE.}

A function $f: \R^m \to \R$ is called \mydef{homogeneous of degree $k$} if $\forall \allocation[ ] \in \R^m, \lambda > 0, f(\lambda \allocation[ ]) = \lambda^k f(\allocation[ ])$.
The set of FMCE of any Fisher market $(\valuation, \budget)$ with continuous, concave, and homogeneous utility functions is equal to the set of Nash equilibria of the \mydef{Eisenberg-Gale min-max game},%
\footnote{This min-max game corresponds to the Lagrangian saddle-point formulation of the Eisenberg-Gale program \cite{gale1989theory, jain2005market}.} 
a convex-concave min-max game between a seller who chooses prices $\price \in \simplex[\numgoods]$ and buyers who collectively choose allocations %\amy{consumptions?} 
$\allocation \in \consumptions$, the joint consumption space. 
The objective function of this game comprises two sums: the first is the logarithmic Nash social welfare of the buyers' utility per budget, i.e., bang-per-buck, while the second is the profit of a fictional auctioneer who sells the goods in the market:
% \amy{this formula was not compiling. it was incomplete. it now compiles, but please complete. thanks.}
%
%\begin{align}
%\label{eq:fisher_market_game}
    $\min_{\price \in \simplex[\numgoods]} \max_{\allocation \in \consumptions} \obj (\price, \allocation; \budget) \doteq \sum_{\buyer \in \buyers} \budget[\buyer] \log \left( \valuation[\buyer](\allocation[\buyer]) \right) + \sum_{\good \in \goods} \left( \price[\good] - \price[\good] 
    \sum_{\buyer \in \buyers}\allocation[\buyer][\good] \right)$.
%\end{align}
%
% Note that for all $\price \in \simplex[\numgoods]$, $\obj (\price, \allocation; \budget)$ is jointly concave in $(\allocation, \budget)$.
% To see this, observe that the first sum in $\obj$, which depends on $(\allocation, \budget)$, corresponds to the negated KL-divergence between the budgets and the utilities of the buyers.
% Since the KL divergence is convex in both arguments \cite{boyd2004convex}, and the KL-divergence is a non-decreasing function in its second argument, the KL divergence between the budgets and the utilities of the buyers is convex in $(\allocation, \budget)$.
% Additionally, for any $(\allocation, \budget) \in \consumptions \times \simplex[\numbuyers]$, $\obj (\price, \allocation; \budget)$ is affine, i.e., convex, \amy{why is affine the same as convex here?} in $\price$.

An \mydef{exchange economy} $(\numbuyers, \numgoods, \valuation, \consendow)$,  $(\valuation, \consendow)$ when clear from context, consists of a finite set of $\numgoods \in \N_+$ goods and $\numbuyers \in \N_+$ consumers (or traders, or buyers).
Each consumer $\buyer \in \buyers$ has a set of possible consumptions $\consumptions[\buyer] \subseteq \mathbb{R}^{\numgoods}_+$, an endowment of divisible goods $\consendow[\buyer] = \left(\consendow[\buyer][1], \dots, \consendow[\buyer][\numgoods] \right) \in \R^\numgoods$, and a utility function $\valuation[\buyer]: \mathbb{R}^{\numgoods } \to \mathbb{R}$.
We define $\consendow \doteq \left(\consendow[1], \hdots, \consendow[\numbuyers] \right)^T$, and assume without loss of generality that there is one unit of supply of each good, i.e., $\sum_{\buyer \in \buyers} \consendow[\buyer] = \ones[\numgoods]$. 
% An exchange market $(\valuation, \budget)$ is said to be \mydef{homothetic} if, for all buyers $\buyer \in \buyers$, $\valuation[\buyer]$ is a continuous and homogeneous of degree 1, i.e., for all $\lambda \in \R_+$ $\valuation[\buyer](\lambda \allocation[\buyer]) = \lambda \valuation[\buyer](\allocation[\buyer])$\footnote{Without loss of generality, complete, transitive, continuous, and homothetic preference relations can be represented via a homogeneous utility function of degree 1, since any homogeneous utility function of degree $k$ can be made homogeneous of degree 1 without affecting the underlying preference relation by passing the utility function through the monotonic transformation $x \mapsto \sqrt[k]{x}$.}.

% \deni{To add somewhere in a non-confusing way, rn I think it is confusing.}
% \sdeni{}{A Fisher economy $(\valuation, \budget)$ is an exchange market $(\numbuyers + 1, \numgoods + 1, \valuation[][\prime], \consendow)$ where the first consumer called the seller is endowed with the first $\numgoods$ goods, i.e., $\forall \good \in \goods$, $\consendow[1][\good] = 1$, and gets utility $\valuation[1][\prime](\allocation[1]) = \allocation[1,][\numgoods + 1]$, while the $\numbuyers$ last consumers called the buyers are only endowed with good $\numbuyers + 1$ such that for all $\buyer \in [1, \numbuyers + 1]$, $\consendow[\buyer][\numgoods + 1] = \budget[\buyer]$ and have utility functions $\valuation[\buyer][\prime](\allocation[\buyer]) = \valuation[\buyer](\allocation[\buyer, -\numgoods + 1])$.}

An \mydef{Arrow-Debreu competitive equilibrium (ADCE)} is a tuple comprising allocations $\allocation \in \R_+^{\numgoods \times \numbuyers}$ and prices $\price \in \simplex[\numgoods]$ s.t.\ 1.~all traders $\buyer \in \buyers$ maximize utility constrained by the value of their endowment: $\allocation[\buyer]^* \in \argmax_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price \leq \consendow[\buyer] \cdot \price} \valuation[\buyer](\allocation[\buyer])$, 2.~the markets clear, meaning 
% \amy{same edits as above!: feasibility and Walras' law}
the allocation is feasible and Walras' law holds, i.e., $\sum_{\buyer \in \buyers} \allocation[\buyer]^*  \leq \ones[\numgoods]$ and $\price^* \cdot \left( \sum_{\buyer \in \buyers} \allocation[\buyer]^*  - \ones[\numgoods] \right) = 0$.

%In the rest of this section, we restrict our attention to exchange markets with homogeneous utility functions for which an ADCE \samy{}{necessarily} exists. 
Our main result concerns \mydef{homothetic} exchange economies, namely those in which utilities functions are homogeneous.
Modulo the homogeneity assumption, the following assumptions are identical to those introduced by \citeauthor{arrow-debreu} \cite{arrow-debreu} to establish the existence of ADCE in exchange economies.
We adopt these assumptions in the sequel.
% \citeauthor{arrow-debreu} also introduce alternative assumptions; our results hold under those assumptions as well. 

\begin{assumption}[Homogeneous Market Assumption]
\label{assum:ad_exist}
Given exchange economy $(\util, \consendow)$, for all consumers $\buyer \in \buyers$, assume 1.~$\util[\buyer]$ is continuous, concave,%
%%% SPACE
%\footnote{Technically speaking, \citeauthor{arrow-debreu} \cite{arrow-debreu} assume payoffs are quasi-concave, a generalization of concavity. Nonetheless, for ease of presentation, we state our results under the stronger assumption of concavity.} 
locally non-satiated, and homogeneous; 2.~$\consumptions[\buyer]$ is non-empty, compact, and convex; and 3.~there exists $\consumption[\buyer] \in \consumptions[\buyer]$, such that $\consumption[\buyer] < \consendow[\buyer]$.
\end{assumption}

%\amy{note to self: existence before observation, so that observation is not vacuous}

The following lemma characterizes a key relationship between the competitive equilibria of Arrow-Debreu exchange economies and those of a particular Fisher market.

\begin{observation}
\label{obs:ad_fisher_eq_equiv}
    $(\allocation^*, \price^*)$ is an %competitive equilibrium 
    ADCE of an exchange economy $(\valuation, \consendow)$ iff it is an FMCE
    %competitive equilibrium
    of the Fisher market $(\valuation, \consendow \price^*)$.
\end{observation}

\vspace{-2.5mm}
%\begin{proof}
\emph{Proof.}
$(\allocation^*, \price^*)$ is an ADCE
%competitive equilibrium 
of the exchange market $(\valuation, \consendow)$ iff
%    \begin{align}
        for all $\buyer \in \buyers$, $\allocation[\buyer]^* \in  \argmax_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*} \valuation[\buyer](\allocation[\buyer])$;
        $\sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^* \leq \ones[\numgoods]$; and 
        $\price^* \cdot \left( \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  - \ones[\numgoods] \right) = 0$
%    \end{align} 
    iff $(\allocation^*, \price^*)$ is an FMCE
    %competitive equilibrium 
    of the Fisher market $(\valuation, \consendow \price^*)$.
%\end{proof}

\if 0
\begin{proof}
    $(\Rightarrow)$
    If $(\allocation^*, \price^*)$ is a competitive equilibrium of the Arrow-Debreu exchange market $(\valuation, \consendow)$, then
    \begin{align}
        \allocation[\buyer]^* \in  \argmax_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*} \valuation[\buyer](\allocation[\buyer]), \forall \buyer \in \buyers,
        \qquad
        \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  \leq \ones[\numgoods],
        \qquad
        \price^* \cdot \left( \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  - \ones[\numgoods] \right) = 0
    \end{align} 
    which correspond to the competitive equilibrium conditions for the Fisher market $(\valuation, \consendow \price^*)$.
    % Similarly, suppose that 
    % However,
    % % \fi 
    % Under \Cref{assum:ad_exist}, the utilities of the consumers are locally non-satiated, which implies that they \sdeni{consume}{spend} \sdeni{their entire budget}{the entire value of their endowment}.
    % As a result, for $\allocation^*$ to be utility maximizing at prices $\price^*$, $\allocation^* \cdot \price^* = \consendow^* \cdot \price^*$ (see, for instance, \cite{mas-colell}). 
    % % \amy{what is $\budget^*$ in this proof? it seems to be unquantified. i guess it will lead to the magic of the leader's objective in the CP. but it has not been adequately explained/motivated here, yet.}
    % Since $(\allocation^*(\budget^*), \price^*(\budget^*))$ is a competitive equilibrium of $(\valuation, \consendow)$, it holds that allocations $\allocation^*(\budget^*)$  are utility maximizing at budgets $\consendow\price^*(\budget^*)$.
    % Hence, by local non-satiation, for all consumers $\buyer \in \buyers$, $\allocation[\buyer]^* \cdot \price^* = \consendow[\buyer] \cdot \price^*(\budget^*)$.
    % Combining these two budget constraints yields \samy{$\budget^* = \consendow \price^*(\budget^*)$}{$\budget^* = \consendow \price^*$}.
    % Thus $(\allocation^*, \price^*)$ is a competitive equilibrium of the Fisher market $(\valuation, \consendow \price^*)$.
    
    $(\Leftarrow)$
    If $(\allocation^*, \price^*)$ is a competitive equilibrium of the Fisher market $(\valuation, \consendow \price^*)$, then
    \begin{align}
    \allocation[\buyer]^* \in \argmax_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price^* \leq \consendow[\buyer] \cdot \price^*} \valuation[\buyer](\allocation[\buyer]), \forall \buyer \in \buyers, \qquad
    \sum_{\buyer \in \buyers} \allocation[\buyer]^* \leq \ones[\numgoods], \qquad
    \price^* \cdot \left( \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  - \ones[\numgoods] \right) = 0
    \enspace ,
    \end{align}
    which correspond to the competitive equilibrium conditions for the Arrow-Debreu economy $(\valuation, \consendow)$.
\end{proof}
\fi

% Define $\obj (\price, \allocation; \budget) = \sum_{\buyer \in \buyers} \budget[\buyer] \log(\frac{\valuation[\buyer](\allocation[\buyer])}{\budget[\buyer]}) + \sum_{\good \in \goods}  \left( \price[\good] - \price[\good] 
    % \sum_{\buyer \in \buyers} \allocation[\buyer][\good] \right)$ which corresponds to the objective of the Fisher market min-max game.

\begin{corollary}
\label{cor:ad_fixed_point}
To find ADCE prices of an exchange economy $(\valuation, \consendow)$, it suffices to find budgets $\budget^* \in \simplex[\numbuyers]$ s.t.\ $\budget^* = \consendow \price^*$ and $\price^*$ are FMCE prices of the Fisher market $(\valuation, \budget^*)$.
\end{corollary}

\if 0

Define the operator $\budgetspace (\budget) \doteq \{\consendow \price \mid \price \in \argmin_{\price \in \simplex[\numgoods]} \max_{\allocation \in \consumptions} \obj (\price, \allocation; \budget) \}$.
\amy{the operator solves for FMCE prices, and then multiplies them by endowments, outputs these as consumers' budgets at these eqm prices.}
\amy{learning dynamic: given budgets (like income), solve for eqm = spend income, observes actual income Ep, adjusts next time period income accordingly.}

Given an exchange economy $(\valuation, \consendow)$, prices $\price^*$ for which the value of the buyers' endowments $\budget^* \doteq \consendow \price^*$ are fixed points of $\budgetspace$, i.e., $\budget^* \in \budgetspace (\budget^*)$, are ADCE prices of $(\valuation, \consendow)$.
By \Cref{obs:ad_fisher_eq_equiv}, such prices are also FMCE prices of $(\valuation, \consendow \price^*)$.
Consequently, if we can find budgets $\budget^* \in \simplex[\numbuyers]$ such that $\budget^* = \consendow \price^*$ and $\price^*$ are FMCE prices of $(\valuation, \budget^*)$, then $\consendow \price^* \in \budgetspace (\consendow \price^*)$, meaning we have also found ADCE prices of $(\valuation, \consendow)$.

\fi

%\deni{This should go in the related works section imo}\amy{i don't agree. it could be repeated in the intro, if you want. but it's purpose here is to motivate/explain the direction we are going with all these definitions. telling the reader why they should be paying attention.}

Prior work has proposed first-order methods to solve Fisher markets by defining a Stackelberg game whose equilibria correspond to FMCE \cite{goktas2021minmax}.
We employ a similar strategy: we solve exchange economies by defining a Stackelberg-Nash game whose SSNE correspond to ADCE.
We call this Stackelberg-Nash game the budget-balance game, and note that it can represent any exchange economy $(\valuation, \consendow)$ with continuous, concave, and homogeneous utility functions.

In the budget-balance game, the leader chooses budgets for the followers, who then choose prices and allocations simultaneously \amy{why did this become a Nash game, instead of a Stackelberg game?} in the Eisenberg-Gale min-max game determined by these budgets.
%%% SPACE
%(\Cref{eq:fisher_market_game}).
The lower-level game is thus a Fisher market, whose set of Nash equilibria is precisely the set of FMCE.
%(Theorem 2, \citeauthor{goktas2022cch} (\citeyear{goktas2022cch})).
The leader's objective is to choose budgets for which $\budget^* = \consendow^* \price$, which by \Cref{cor:ad_fixed_point} yield a competitive equilibrium in $(\valuation, \consendow)$. 

%\amy{want to find $\budget^*$ s.t.\ $\budget^* = \consendow \price^*(\budget^*)$.}

\begin{definition}[Budget-Balance Game]\label{def:budget_balance}
Given an exchange economy $(\valuation, \consendow)$, a \mydef{budget-balance game} is a Stackelberg-Nash game $(3, \outerset, \innerset, \util)$ with one leader and two followers, with leader action space $\outerset \doteq \simplex[\numbuyers]$, and action spaces $\innerset[1] \doteq \simplex[\numgoods]$ and $\innerset[2] \doteq \consumptions$ for the two followers. 
In this game, the leader first chooses a budget $\budget \in \simplex[\numbuyers]$ for each of the followers, after which the first follower chooses prices $\price \in \simplex[\numgoods]$ and the second follower chooses allocations $\allocation \in \consumptions$, simultaneously.
%After all players choose their actions, the players receive the following payoffs:
The payoffs are:
%%% SPACE
%as follows:
%\begin{align}
$\util[0](\budget, \price, \allocation) = -\frac{1}{2}\left\| \budget - \consendow \price\right\|_2^2$,
$\util[1](\budget, \price, \allocation) = - \obj (\budget, \price, \allocation)$, and 
$\util[2](\budget, \price, \allocation) = \obj (\budget, \price, \allocation)$.
%\end{align}
\end{definition}

% \begin{theorem}
\begin{restatable}{theorem}{thmadssneequiv}
\label{thm:ad_ssne_equiv}
Given an exchange economy $(\valuation, \consendow)$ that satisfies Assum.~\ref{assum:ad_exist},
% }{} \amy{can drop, i think, if we point out somewhere earlier that we've adopted this assumption in what follows.}
$(\budget^*, \price^*, \allocation^*)$ is an SSNE of the budget-balance game $(3, \outerset, \innerset, \util)$ associated with $(\valuation, \consendow)$ iff $(\allocation^*, \price^*)$ is an ADCE of $(\valuation, \consendow)$. 
% \end{theorem}
\end{restatable}
\if 0
%%% APPENDIX
\begin{proof}
    $(\Rightarrow):$ Assume $(\budget^*, \allocation^*, \price^*)$ is a SSNE of the budget-balance game $(3, \outerset, \innerset, \util)$ associated with the homothetic exchange economy $(\valuation, \consendow)$. 
    Then, $(\allocation^*, \price^*)$ is a FMCE of the homothetic Fisher market $(\valuation, \budget^*)$, since $(\allocation^*, \price^*)$ is a Nash equilibrium of the associated Fisher market min-max game. 
    
    % \samy{By way of contradiction, assume $\budget^* \neq \consendow \price^*$.}{} \amy{i'm not quite seeing how this contradicts $(\allocation^*, \price^*)$ being an ADCE of $(\valuation, \consendow)$. but i am not sure we need this, anyway.}
    
    Under \Cref{assum:ad_exist}, an ADCE $(\allocation^\prime, \price^\prime)$ exists.
    By \Cref{obs:ad_fisher_eq_equiv}, $(\allocation^\prime, \price^\prime)$ is a FMCE of $(\valuation, \consendow \price^\prime)$, and hence a Nash equilibrium of the associated Eisenberg-Game min-max game at budgets $\budget^\prime = \consendow \price^\prime$.
    Now, setting $\budget^\prime = \consendow \price^\prime$, it follows that $(\budget^\prime, \allocation^\prime, \price^\prime)$ is a SSNE of $(3, \outerset, \innerset, \util)$, because the leader's payoff at this SSNE is $0$, which is the lower bound of its value.
    %\amy{this part of the argument is the same as in the other direction.} 
    
    However, if the leader's payoff at any SSNE is equal to 0, then it must be so at any other SSNE, since the equilibrium payoff of the leader is unique. That is, we must have that that $\budget^* = \consendow \price^*$. Since $(\allocation^*, \price^*)$ is a FMCE of $(\valuation, \consendow \price^*)$, by \Cref{obs:ad_fisher_eq_equiv}, $(\allocation^*, \price^*)$ is likewise an ADCE of $(\valuation, \consendow)$.

    $(\Leftarrow)$: Assume $(\allocation^*, \price^*)$ is an ADCE of the homothetic exchange economy $(\valuation, \consendow)$. Then, by \Cref{obs:ad_fisher_eq_equiv}, $(\allocation^*, \price^*)$ is a FMCE of the Fisher market $(\valuation, \consendow \price^*)$. Hence, $(\allocation^*, \price^*)$ is a Nash equilibrium of the associated Eisenberg-Gale min-max game at budgets $\budget^* \doteq \consendow \price^*$. However, at budgets $\budget^* = \consendow \price^*$, the payoff of the leader is minimized in the budget-balance game $(3, \outerset, \innerset, \util)$, i.e., its value is the lower bound, namely 0. As the leader's action is optimal, and the followers' actions comprise a Nash equilibrium, $(\budget^*, \allocation^*, \price^*)$ is a SSNE of the budget-balance game.
\end{proof}
\fi

\amy{add motivating text: e.g.,}

Having reduced ADCE in homothetic exchange economies to SSNE in budget-balance games, a class of Stackelberg-Nash games, it remains to apply our method 
%(\Cref{alg:npam}} 
to solving these games. 
\sdeni{}{However, 
%as mentioned previously, 
falling short of the leader's action being affine in the followers' payoff, the exploitability is not guaranteed to be convex in all players' actions in the convex-concave min-max lower-level game.}
%%% FIX ME !!!
\amy{add more about: however, convexity, weak convexity, etc., to motivate the rest of this section?!}

Given a budget-balance Stackelberg-Nash game together with the leader's choice of budgets $\budget$, the follower cumulative regret of the lower-level Eisenberg-Gale min-max game is given by: $\cumulregret[\budget] ((\price, \allocation), (\otherprice, \otherallocation); \budget) \doteq \obj (\otherprice, \otherallocation; \budget) - \obj (\price, \allocation; \budget)$.
\amy{i added a $\budget$ subscript to $\cumulregret$. i think you need it for consistency.}\deni{Consistency with what? the regularized cumulative regret? Becuse this is now in conflict with previous section's notation.}
\if 0
\begin{align}
&\obj (\otherprice, \otherallocation; \budget) - \obj (\price, \allocation; \budget) \\
=& \sum_{\buyer \in \buyers} \budget[\buyer] \log \left( \valuation[\buyer](\otherallocation[\buyer]) \right) + \sum_{\good \in \goods} \left( \otherprice[\good] - \otherprice[\good] 
    \sum_{\buyer \in \buyers} \otherallocation[\buyer][\good] \right) - \sum_{\buyer \in \buyers} \budget[\buyer] \log \left( \valuation[\buyer](\allocation[\buyer]) \right) + \sum_{\good \in \goods} \left( \price[\good] - \price[\good] 
    \sum_{\buyer \in \buyers}\allocation[\buyer][\good] \right)
\end{align}
\fi
Under \Cref{assum:ad_exist}, this cumulative regret is concave in $(\otherprice, \otherallocation)$ and convex in $(\price, \allocation)$, but it is not convex in $(\budget, \price, \allocation)$. 
However, if $\consumptions$ is bounded away from zero, then $\obj$ is twice continuously differentiable, in which case, the leader-regularized cumulative regret $\regulcumulregret[\budget]$ is Lipschitz-smooth over $\simplex[\numgoods] \times \consumptions \times \simplex[\numgoods] \times \consumptions$,
%\amy{good use of ``over''. clarifying.} 
and further, by \Cref{lemma:reg_expl_prop}, the leader-regularized exploitability $\regulexploit[\budget]$ is convex in $(\budget, \price, \allocation)$. 

Nonetheless, 
%%% FIX ME !!!
as mentioned previously, \amy{please remind me where? thanks.}\deni{Line 401.}\amy{line numbers changed before i saw this!}
using an entropy rather than Euclidean regularizer can make it easier to achieve convexity in $(\budget, \price, \allocation)$.
%%% FIX ME !!!
\amy{but we already achieved convexity, so i am not sure i follow?}
We thus define the leader-regularized cumulative regret as the cumulative regret with an additional entropy term for the budgets:
%%% FIX ME !!!
\amy{why do you add the regularization term only once? that is, why do you add it to $\regulcumulregret[\budget]((\price, \allocation), (\otherprice, \otherallocation); \budget)$ instead of to $\obj (\otherprice, \otherallocation; \budget)$ and $\obj (\price, \allocation; \budget)$? if you added it to $\obj$, you would have what i've written below in red, i think. but this term is not negated, which may be why you cannot do it this way?}\deni{The regularization is added to the cumulative regret not the payoffs, if we add it to the payoffs the regularization terms cancel out for the cumulative regret.} \amy{i'm not seeing that. you could incorporate each of the regularization into each of the $\val[\buyer]$ terms, rather than cancel them out.}
$\regulcumulregret[\budget]((\price, \allocation), (\otherprice, \otherallocation); \budget) \doteq \cumulregret[\budget]((\price, \allocation), (\otherprice, \otherallocation); \budget) + \sum_{\buyer \in \buyers} \budget[\buyer] \log(\budget[\buyer]) =$
%\begin{align}
    $\sum_{\buyer \in \buyers} \budget[\buyer] \log \left( \valuation[\buyer](\otherallocation[\buyer]) \right) + \sum_{\good \in \goods} \left( \otherprice[\good] - \otherprice[\good] 
    \sum_{\buyer \in \buyers} \otherallocation[\buyer][\good] \right) - \sum_{\buyer \in \buyers} \budget[\buyer] \log \left( \frac{\valuation[\buyer](\allocation[\buyer])}{\budget[\buyer]} \right) + \sum_{\good \in \goods} \left( \price[\good] - \price[\good] 
    \sum_{\buyer \in \buyers}\allocation[\buyer][\good] \right)$.
    %%% FIX ME !!!
    \amy{$\samy{}{\sum_{\buyer \in \buyers} \budget[\buyer] \log \left( \frac{\valuation[\buyer](\otherallocation[\buyer])}{\budget[\buyer]} \right) + \sum_{\good \in \goods} \left( \otherprice[\good] - \otherprice[\good] \sum_{\buyer \in \buyers} \otherallocation[\buyer][\good] \right) - \sum_{\buyer \in \buyers} \budget[\buyer] \log \left( \frac{\valuation[\buyer](\allocation[\buyer])}{\budget[\buyer]} \right) + \sum_{\good \in \goods} \left( \price[\good] - \price[\good] \sum_{\buyer \in \buyers}\allocation[\buyer][\good] \right)}$}
%\end{align}

Under \Cref{assum:ad_exist}, the leader-regularized cumulative regret $\regulcumulregret[\budget]$ is 
%%% FIX ME !!!
convex in $(\budget, \price, \allocation)$, for all $(\otherprice, \otherallocation) \in \simplex[\numgoods] \times \consumptions$. 
The convexity of the first two and the last terms is straightforward, since these terms are linear, fixing $(\budget, \price, \allocation)$.
%%% FIX ME !!!
\amy{i'm not seeing this. let's slow down. (too much info in one sentence.) last term is fine. it is a constant if $(\budget, \price, \allocation)$ is fixed. second term? not sure. first term, linear in $\budget$, but not in $\otherallocation$.}
To see the convexity of the third term, observe that it corresponds to the negated KL-divergence between the budgets and the utilities of the buyers, which is concave in both arguments; since the negated KL divergence is non-decreasing
%%% FIX ME !!!
% \amy{non-decreasing?} 
in its second argument, namely $\allocation[\buyer]$, its composition with a concave utility function is concave; hence the negation of this term is convex in $(\budget, \allocation)$.
% Since the KL divergence is convex in both arguments \cite{boyd2004convex}, and the KL-divergence is a non-decreasing function in its second argument, the KL divergence between the budgets and the utilities of the buyers is convex in $(\allocation, \budget)$.
%
The following corollary now follows from \Cref{thm:ad_ssne_equiv}.

%%% SPACE
%using this entropy-regularized definition of leader cumulative regret.

% \begin{corollary}
\begin{restatable}{corollary}{corrconvexad}
    There exists an $\varepsilon \geq \log(\numbuyers)$ \amy{is this the sense in which we are approximate?} s.t.\ the solutions to the following convex program correspond to the ADCE of $(\valuation, \consendow)$:
\if 0
    %\begin{align}
        $\min_{(\budget, \price, \allocation) \in \simplex[\numbuyers] \times \simplex[\numgoods] \times \consumptions,  \max\limits_{\otherprice, \otherallocation \in \consumptions} \regulcumulregret[\budget]((\price, \allocation), (\otherprice, \otherallocation); \budget) \leq \varepsilon} \frac{1}{2}\left\| \budget - \consendow \price\right\|_2^2$,
        %\enspace ,
    %\end{align}
\fi
    %\begin{align}
        $\min_{(\budget, \price, \allocation) \in \simplex[\numbuyers] \times \simplex[\numgoods] \times \consumptions, \regulexploit (\allocation, \price; \budget) \le \varepsilon} \frac{1}{2} \left\| \budget - \consendow \price\right\|_2^2$, 
        %\enspace ,
    %\end{align}    
where $\regulexploit (\allocation, \price; \budget) \doteq \max\limits_{\otherprice, \otherallocation \in \consumptions} \regulcumulregret[\budget]((\price, \allocation), (\otherprice, \otherallocation); \budget)$.
% \end{corollary}
\end{restatable}
    
\if 0
%%% APPENDIX
\begin{proof}
    By \Cref{obs:ssne_max}, we can express the SSNE of the budget-balance game as the following maximization problem, where $\max\limits_{\allocation^\prime \in \consumptions} \obj (\price, \allocation^\prime, \budget) - \min\limits_{\price^\prime \in \simplex[\numgoods]} \obj (\price^\prime, \allocation, \budget)$ describes the \samy{}{follower} exploitability in the lower-level Eisenberg-Gale min-max game:\amy{i think the first of these should be a maximization problem, not a min}
%
\begin{align}
\label{eq:final convex program}
    \min_{\substack{(\budget, \price, \allocation) \in \simplex[\numbuyers] \times \simplex[\numgoods] \times \consumptions\\ \max\limits_{\otherprice, \otherallocation \in \consumptions} \regulcumulregret[\budget]((\price, \allocation), (\otherprice, \otherallocation); \budget) \leq \varepsilon}} - \frac{1}{2}\left\| \budget - \consendow \price\right\|_2^2
    &= \min_{\substack{(\budget, \price, \allocation) \in \simplex[\numbuyers] \times \simplex[\numgoods] \times \consumptions\\ \max\limits_{\otherprice, \otherallocation \in \consumptions} \regulcumulregret[\budget]((\price, \allocation), (\otherprice, \otherallocation); \budget) \leq \varepsilon}} \frac{1}{2}\left\| \budget - \consendow \price\right\|_2^2
\end{align}

\sdeni{}{\Cref{eq:final convex program} is a convex optimization problem with convex constraints.
In particular, the \samy{}{follower} exploitability, i.e., $\regulexploit (\allocation, \price; \budget) \doteq \max\limits_{\otherprice, \otherallocation \in \consumptions} \regulcumulregret[\budget]((\price, \allocation), (\otherprice, \otherallocation); \budget)$, is convex in $(\budget, \allocation, \price)$. To see this, simply notice that $\obj$ is convex } \amy{you trail off...}
\end{proof}
\fi

% \begin{lemma}\label{lemma:fixed_point_ad}
% % and suppose that \Cref{assum:ad_exist} holds 
% % Let $(3, \outerset, \innerset, \util)$ be the budget balance game associated with $(\numbuyers, \numgoods, \valuation, \consendow)$. 
% For any budget $\budget \in \simplex$, let $(\allocation^*(\budget), \price^*(\budget))$ be the competitive equilibrium of the homothetic Fisher market $(\valuation, \budget), i.e., \price^*(\budget) \in  \min\limits_{\price \in \simplex[\numgoods]} \max\limits_{\allocation \in \consumptions} \obj (\price, \allocation, \budget)$ and $\allocation^*(\budget) \in \argmax\limits_{\allocation \in \consumptions} \obj (\price^*(\budget), \allocation, \budget)$. 
% Consider a homothetic exchange economy $(\valuation, \consendow)$ and suppose that \Cref{assum:ad_exist} holds. Then, $(\price^*(\budget^*), \allocation^*(\budget^*))$ is a competitive equilibrium of the Arrow-Debreu economy $(\valuation, \consendow)$ iff $\budget^* = \consendow \price^*(\budget^*)$.
% \end{lemma}
% \begin{proof}
%     $(\Rightarrow)$
%     Since $(\allocation^*(\budget^*), \price^*(\budget^*))$ is a competitive equilibrium of the Fisher market $(\valuation, \budget^*)$ then allocations $\allocation^*(\budget^*)$  are utility maximizing at budgets $\budget^*$, i.e., for all buyers $\buyer \in \buyers$:
%     \begin{align}
%         \allocation[\buyer]^*(\budget^*) \in  \argmax_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price^*(\budget^*) \leq \budget^*} \valuation[\buyer](\allocation[\buyer])
%     \end{align}
%     However, under \Cref{assum:ad_exist}, the utilities of the buyers are locally non-satiated. As a result, for $\allocation^*$ to be utility maximizing, we must have that $\allocation[\buyer]^*(\budget^*) \cdot \price^*(\budget^*) = \budget^*$ (see for instance \cite{mas-colell}).
%     Similarly, since $(\allocation^*(\budget^*), \price^*(\budget^*))$ is a competitive equilibrium of $(\numbuyers, \numgoods, \valuation, \consendow)$, we also have that allocations $\allocation^*(\budget^*)$  are utility maximizing at budgets $\consendow\price^*(\budget^*)$. Hence, by local non-satiation, we must have that for all consumers $\buyer \in \buyers$, $\allocation[\buyer]^*(\budget^*) \cdot \price^*(\budget^*) = \consendow[\buyer] \cdot \price^*(\budget^*)$. Combining the two budget constraint equations for all buyers, we then obtain $\budget^* = \consendow \price^*(\budget^*)$.
    
%     $(\Leftarrow)$
%     Since $(\allocation^*(\budget^*), \price^*(\budget^*))$ is a competitive equilibrium of the Fisher market $(\valuation, \budget^*)$ and $\budget^* = \consendow \price^*(\budget^*)$, we have that:
%     \begin{align}
%         \allocation[\buyer]^* \in \argmax_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price \leq \budget[\buyer]^*} \valuation[\buyer](\allocation[\buyer]) = \argmax_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price \leq \consendow[\buyer] \cdot \price^*} \valuation[\buyer](\allocation[\buyer])
%     \end{align}
%     \begin{align}
%         \sum_{\buyer \in \buyers} \allocation[\buyer]^* &\leq \ones[\numgoods]\\
%         \price^* \cdot \left( \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  - \ones[\numgoods] \right) &= 0
%     \end{align}
%     which correspond to the competitive equilibrium conditions for the Arrow-Debreu economy $(\valuation, \consendow)$.
% \end{proof}

% \begin{lemma}
%     Under \Cref{assum:ad_exist}, the leader's utility at a SSNE $(\budget^*, \allocation^*, \price^*)$ of the budget balance game $(3, \outerset, \innerset, \util)$ associated with the homothetic exchange economy $(\valuation, \consendow)$ is equal to $0$, i.e., $\left\| \budget^* - \consendow \price^*\right\|_2^2$, iff $(\allocation^*, \price^*)$ is a competitive equilibrium $(\numbuyers, \numgoods, \valuation, \consendow)$. 
% \end{lemma}

% \begin{theorem}
% Consider a homothetic exchange economy $(\valuation, \consendow)$ and suppose that \Cref{assum:ad_exist} holds. Consider the budget balance game $(3, \outerset, \innerset, \util)$ associated with $(\numbuyers, \numgoods, \valuation, \consendow)$. Then, $(\budget^*, \price^*, \allocation^*)$ is an SSNE of the budget balance game $(3, \outerset, \innerset, \util)$ iff $(\allocation^*, \price^*)$ is a competitive equilibrium of $(\numbuyers, \numgoods, \valuation, \consendow)$.
% \end{theorem}
% \begin{proof}
%     $(\Rightarrow)$:
%     Let $(\budget^*, \allocation^*, \price^*)$ be an SSNE of the budget balance game $(3, \outerset, \innerset, \util)$. 
%     Note that under \Cref{assum:ad_exist}, an Arrow-Debreu competitive equilibrium $(\allocation^\prime, \price^\prime)$ exists. Note that $(\allocation^\prime, \price^\prime)$ is a Nash equilibrium for the followers under budgets $\budget^\prime = \consendow \price^*\prime$ 
    
%     Since $\nicefrac{1}{2} \left\| \budget^* - \consendow\price^*\right\|_2^2 = 0$, we must have that $\budget^* = \price^*$. Additionally, by the constraints of the optimization problem, we have that $(\price^*, \allocation^*)$ is a Nash equilibrium of the convex-concave min-max game $\min_{\price \in \simplex[\numgoods]} \max_{\allocation \in \consumptions} \obj (\price, \allocation, \budget^*)$. In other words,  $(\price^*, \allocation^*)$ is competitive equilibrium of the Fisher market$(\valuation, \budget^*)$ meaning that:
%     \begin{align}
%         \allocation[\buyer]^* \in \argmax_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price \leq \budget[\buyer]^*} \valuation[\buyer](\allocation[\buyer]) = \argmax_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price \leq \consendow[\buyer] \cdot \price^*} \valuation[\buyer](\allocation[\buyer])
%     \end{align}
%     \begin{align}
%         \sum_{\buyer \in \buyers} \allocation[\buyer]^* &\leq \ones[\numgoods]\\
%         \price^* \cdot \left( \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  - \ones[\numgoods] \right) &= 0
%     \end{align}
%     $(\Leftarrow)$:
%     Since $(\price^*, \allocation^*)$ is competitive equilibrium of the Exchange market we have that $(\valuation, \consendow)$ meaning that:
%     \begin{align}
%         \allocation[\buyer]^* \in \argmax_{\allocation[\buyer] \in \consumptions[\buyer]: \allocation[\buyer] \cdot \price \leq \consendow[\buyer] \cdot \price^*} \valuation[\buyer](\allocation[\buyer])
%     \end{align}
%     \begin{align}
%         \sum_{\buyer \in \buyers} \allocation[\buyer]^* &\leq \ones[\numgoods]\\
%         \price^* \cdot \left( \sum_{\buyer = 1}^{\numagents} \allocation[\buyer]^*  - \ones[\numgoods] \right) &= 0
%     \end{align}
% \end{proof}

==> bayesian.tex <==
\subsubsection{Bayesian Games}
\deni{Makes distributions bold.}
A \mydef{Bayesian game} \cite{harsanyi1968bayesian} $\bgames \doteq (\numplayers, \numactions, \numtypes, \typespace, \typedistrib, \param, \actionspace, \util)$ is a simultaneous-move game which consists of $\numplayers \in \N_+$ players each of whom is characterized by a type space $\typespace[\player] \subset \R^\numtypes$. \amy{characterized by a type in a type space, n'est-ce pas?}\deni{I think these comments are not relevant now that we are reverting to the classical Bayesian game setting no?}\amy{yes, maybe not.}
The players share a \mydef{common prior distribution} \amy{the players don't need a common prior if they see each other's types. they only need this in the independent case, where they see only their own type.}
\amy{the setup does not feel very Bayesian to me. it feels stochastic. like there is a distribution over complete-info games, as determined by the prior and the types, both(?) of which the players observe.} $\typedistrib[\param] \sim \simplex(\typespace)$ over the the \mydef{joint type space} $\typespace \doteq \bigtimes_{\player \in \players} \typespace[\player]$ defined by a \mydef{parameter} $\param \in \params$ coming from a parameter space $\params \subset \R^{\numparams}$.\deni{Make sure ``numparams'' dimensionality does not conflict with other var. def'n}
Each player $\player \in \players$ takes an action $\action[\player] \in \actionspace[\player]$ from its action space $\actionspace[\player] \subset \R^{\numactions}$, and receives a payoff $\util[\player](\action; \type)$ given by the payoff function $\util[\player]: \actionspace \times \typespace \to \R$. We denote the players' \mydef{joint action space} by $\actionspace \doteq \bigtimes_{\player \in \players} \actionspace[\player] \subset \R^{\numplayers \numactions}$ and the vector-valued function of all players' utilities $\util(\action; \type) \doteq \left( \util[\player](\action; \type) \right)_{\player \in \players}$.


% and $\typespace \doteq \bigtimes_{\player \in \players} \typespace[\player] \subset \R^{\numplayers \numtypes}$, and refer to any collection of actions $\action = (\action[1], \hdots, \action[\numplayers]) \in \actionspace$ and types $\type = (\type[1], \hdots, \type[\numplayers]) \in \typespace$ as an \mydef{action profile} and \mydef{type profile} respectively.
% At each time-step $\iter = 0, 1, \hdots$, each player $\player \in \players$ takes an action $\inner[\player][][][\iter] \in \innerset[\player](\context[\iter])$ from an action space $\innerset[\player](\context[\iter]) \subset \actionspace[\player]$\footnote{Going forward, for simplicity, without loss of generality, we drop the dependence of the action space $\innerset[\player]$ on the context $\context$ and take for all player $\player \in \players$, $\innerset[\player] \doteq \actionspace[\player]$.} simultaneously observe a \mydef{context} $\typerv[][\iter] \sim \initcontexts$, i.e., a type profile drawn from a distribution $\initcontexts \in \simplex(\typespace)$ over the set of types. Each player $\player \in \players$ , it takes an action $\inner[\player][][][\iter] \in \innerset[\player](\context[\iter])$ from an action space $\innerset[\player](\context[\iter]) \subset \actionspace[\player]$\footnote{Going forward, for simplicity, without loss of generality, we drop the dependence of the action space $\innerset[\player]$ on the context $\context$ and take for all player $\player \in \players$, $\innerset[\player] \doteq \actionspace[\player]$.}

% Once player $\player \in \players$ has observed the realized contexts $\context[\iter]$, it takes an action $\inner[\player][][][\iter] \in \innerset[\player](\context[\iter])$ from an action space $\innerset[\player](\context[\iter]) \subset \actionspace[\player]$\footnote{Going forward, for simplicity, without loss of generality, we drop the dependence of the action space $\innerset[\player]$ on the context $\context$ and take for all player $\player \in \players$, $\innerset[\player] \doteq \actionspace[\player]$.} and receive reward $\reward[\player](\context, \inner; \type[\player])$ given by a reward function $\reward[\player]: \contexts \times \innerset \times \typespace \to \R$. For a given context, action profile, and type profile tuple, we denote the vector of all  players utilities by $(\context, \action, \type) \mapsto \reward(\context, \action; \type)$  

A Bayesian game is \mydef{continuous} if for all $\type \in \contexts$, $\util(\action; \type)$ is continuous in $\action$ and $\actionspace$ is non-empty and compact.
A Bayesian game is \mydef{concave} if in addition to being continuous, for all types $\type \in \typespace$ and for all players $\player \in \players$, $\util[\player](\action; \type)$ is concave in $\action[\player]$ and $\actionspace[\player]$ is convex.

% A \mydef{joint strategy profile} $\strat: \typespace \to \actionspace$ is a mapping from the joint type space to the joint action space s.t.\ $\strat[\player](\type) \in \actionspace[\player]$ denotes the action played by player $\player$ under type profile $\type \in \typespace$. 
An \mydef{strategy} 
% \deni{Decide if we want discuss the whole decentralized/centralized issue} \deni{I think yes?}
$\strat[\player]: \typespace[\player] \to \actionspace[\player]$ for a player $\player \in \players$, is a mapping from player $\player$'s type to an action s.t. $\strat[\player](\type[\player]) \in \actionspace[\player]$ denotes the action played by player $\player$ when it is of type $\type[\player]$. 
A \mydef{strategy profile} $\strat \doteq \left( \strat[1], \hdots, \strat[\numplayers]\right)$ is a collection of independent strategies, one-per-player, s.t. for any type profile $\type \in \typespace$, $\strat(\type) \in \actionspace$ denotes the action profile played by the players.
% \amy{i think you need a different letter for independent strategy profiles. maybe $\tau$. overloading with $\sigma$ will probably be too confusing (and you can always change the macro later if it isn't).}

An \mydef{ex-ante $\varepsilon$-Bayesian Nash equilibrium} 
% \amy{maybe parameterized instead of Bayesian}\deni{We said no!} 
($\varepsilon$\mydef{-BNE}) is a strategy profile $\strat[][][*] \in \actionspace^\typespace$ s.t.\ for all players $\player \in \players$ and strategy profiles $\strat \in \actionspace^\typespace$, $\Ex_{\typerv \sim \typedistrib[\param]} \left[ \util[\player] (\strat[][][*](\typerv); \typerv)\right] \geq \Ex_{\typerv \sim \typedistrib[\param]} \left[ \util[\player] (\strat[\player][][](\typerv), \strat[-\player][][*] (\typerv); \typerv)\right] - \varepsilon$. 
A $\varepsilon$-ex-post Nash equilibrium ($\varepsilon$-EPNE) is a strategy profile $\strat[][][*] \in \actionspace^\typespace$ s.t. for all players $\player \in \players$, types $\type \in \typespace$, and strategy profiles $\strat \in \actionspace^\typespace$, $\util[\player](\strat[][][*](\type); \type) \geq \util[\player](\strat[\player][][](\type), \strat[-\player][][*](\type); \type) - \varepsilon$. 
A $0$-BNE and $0$-EPNE are simply called BNE and EPNE, respectively.
For concave games, a BNE is guaranteed to exist, while EPNE are not guaranteed exist.%
% \footnote{Traditionally, BNE and EPNE are only defined for independent strategies, in which case EPNE may not exist. Our more general definition applies to strategies that depend on all players' types. \amy{again, it doesn't feel very ex-post.}} 

\deni{We have to define the set of Nash equilibria and EPNE?} \deni{Update: Maybe not}

% \deni{Ignore next para, Old def'n, to remove, keeping it for visual reminder}
% An \mydef{ex-ante $\varepsilon$-Bayesian Nash equilibrium} (joint $\varepsilon$\mydef{-BNE}) is a strategy profile $\strat[][][*] \in \actionspace^\typespace$ s.t. for all players $\player \in \players$ and strategy profiles $\strat \in \actionspace^\typespace$, $\Ex_{\typerv \sim \typedistrib} \left[ \util[\player](\strat[][][*](\typerv); \typerv)\right] \geq \Ex_{\typerv \sim \typedistrib} \left[ \util[\player](\strat[\player][][](\typerv[\player]), \strat[-\player][][*](\typerv[-\player]); \typerv)\right]$. A $\varepsilon$-ex-post Nash equilibrium ($\varepsilon$-EPNE) is a strategy profile $\strat[][][*] \in \actionspace^\typespace$ s.t. for all players $\player \in \players$, types $\type \in \typespace$ and strategy profiles $\strat \in \actionspace^\typespace$, $\util[\player](\strat[][][*](\type); \type) \geq \util[\player](\strat[\player][][](\type[\player]), \strat[-\player][][*](\type[-\player]); \type)$.

% \amy{BNE seems different to me, b/c i don't think $\strat[][][*](\type) = (\strat[\player][][*](\type[\player]), \strat[-\player][][*](\type[-\player]))$. i think it might equal $(\strat[\player][][*](\type), \strat[-\player][][*](\type))$, in which case you have $\util[\player](\strat[][][*](\type); \type) = \util[\player](\strat[\player][][*](\type), \strat[-\player][][*](\type); \type)$ not $\util[\player](\strat[][][*](\type); \type) = \util[\player](\strat[\player][][*](\type[\player]), \strat[-\player][][*](\type[-\player]); \type)$. in the former case, parameters are known to all---it is a complete-info game; in the latter, players know only their own parameters, which is very different from an info-theoretic point of view (so it feels like we are comparing apples to oranges).}

% A \mydef{(Markov or stationary) policy} \cite{maskin2001markov} for player $\player \in \players$, $\policy[\player]: \contexts \to \innerset[\player]$ is a mapping from contexts to actions such that $\policy[\player](\context) \in \innerset[\player]$ denotes the action taken by player $\player$ when it observes context $\context$. We define a \mydef{policy profile} as the collection of policies, i.e., $\policy = (\policy[1], \hdots, \policy[\numplayers]) : \contexts \to \innerset$ such that $\policy(\context) \in \innerset$ denotes the action profile played by the players under context $\context \in \contexts$. The goal of all players $\player \in \players$ is to play a policy $\policy[\player][][*] \in \innerset[\player]^\context$ which maximizes their \mydef{expected cumulative payoff} $\util[\player](\policy[\player], \policy[-\player]; \type[\player]) \doteq \Ex_{\contextrv \sim \initcontexts} \left[ \reward[\player](\contextrv, \policy[\player](\contextrv), \policy[-\player](\contextrv); \type[\player])\right]$. 
% % 


% A \mydef{$\varepsilon$-subgame perfect Nash equilibrium ($\varepsilon$-SPNE)} of a contextual game is a policy profile $\policy[][][*] \in \innerset^\contexts$ such that for all player $\player \in \players$ and for all contexts $\context \in \contexts$,  $\reward[\player](\context, \policy[][][*](\context); \type[\player]) \geq \reward[\player](\policy[\player](\context), \policy[-\player][][*](\context); \type[\player]) - \varepsilon$. A $0$-SPNE is called a \mydef{subgame perfect Nash equilibrium (SPNE)}. A SPNE is guaranteed to exist in concave contextual games. Additionally, note that when the context space is a singleton, then the SPNE of contextual game simply reduce to the NE of the game played at that context. Further, notice that the SPNE of contextual games with different context distributions are all the same.

% \deni{Ex-ante definition is commented out below. Might want to make the introduction of the type inside the paranthesis not as a superscript.}

\deni{Need to make this a function of the parameter distribution and not a function of the parameter, and us the same expectation overload as the Markov game paper.}
Fixing the payoff functions of the players $\util$, for any type $\type \in \typespace$, we define the 
% \mydef{regret} $\regret[][\util]: \actionspace \times \actionspace \to \R^\numplayers$ for playing an action profile $\action$ as compared to another action profile $\otheraction$, as follows: for all followers $\player \in \players$,
% $\regret[\player][](\action, \otheraction; \outer) = \util[\player](\outer, (\otheraction[\player], \action[-\player])) - \util[\player](\outer, \action)$. The 
\mydef{cumulative regret}, $\cumulregret[][]: \actionspace \times \actionspace \times \typespace \to \R$ between two action profiles $\action \in \actionspace$ and $\otheraction \in \actionspace$ across all players in a game as $\cumulregret[][](\action, \otheraction; \type) = \sum_{\player \in \players} \util[\player](\otheraction[\player], \action[-\player]; \type) - \util[\player](\action; \type)$.
Further, the \mydef{exploitability} or (Nikaido-Isoda potential function \cite{nikaido1955note}) of an action profile $\action \in \actionspace$ is defined as 
$\exploit[][](\action; \type) = \max_{\otheraction \in \actionspace} \cumulregret[][](\action, \otheraction; \type)$ \cite{goktas2022exploit}. 
Overloading notation,
for any common prior distribution parameter $\param \in \params$, we define the \mydef{ex-ante cumulative regret} at any given type profile $\type \in \typespace$, $\cumulregret[][\param]: \actionspace^\typespace \times \actionspace^\typespace \to \R$ between two strategy profiles $\strat \in \actionspace^\typespace$ and $\otherstrat \in \actionspace^\typespace$ across all players as $\cumulregret[][\param](\strat, \otherstrat) = \sum_{\player \in \players} \left( \Ex_{\typerv \sim \typedistrib[\param]} \left[ \util[\player](\otherstrat[\player][][](\typerv[\player]), \strat[-\player][][](\typerv[-\player]); \typerv)\right] -\Ex_{\typerv \sim \typedistrib[\param]} \left[ \util[\player](\strat(\typerv); \typerv)\right] \right)$.
Further, the \mydef{ex-ante exploitability} or (Nikaido-Isoda potential function \cite{nikaido1955note}) of a strategy profile $\strat \in \actionspace^\typespace$ is defined as 
$\exploit[][\param](\strat) = \max_{\otherstrat \in \actionspace^\typespace} \cumulregret[][\param](\strat, \otherstrat)$ \cite{goktas2022exploit}. We note that for all $\strat \in \actionspace^\typespace$, $\exploit[][\param](\strat) \geq 0$, and $\strat[][][*]$ is a BNE of $\game$ iff $\exploit[][\param](\strat[][][*]) = 0$. 
% For
% for any type profile $\type \in \typespace$,
% we define the \mydef{ex-post cumulative regret} and the \mydef{ex-post exploitability} respectively as 
% $\cumulregret[][\type](\strat, \otherstrat) \doteq \sum_{\player \in \players} \left[ \util[\player](\otherstrat[\player][][](\type[\player]), \strat[-\player][][](\type[-\player]); \type) - \util[\player](\strat(\type); \type) \right]$
% $\cumulregret[][] (\action, \otheraction; \type) = \sum_{\player \in \players} \util[\player] (\otheraction[\player], \action[-\player]; \type) - \util[\player] (\action; \type)$
% and $\exploit[][](\strat; \type) \doteq \max_{\otherstrat \in \actionspace} \cumulregret[][] (\strat, \otherstrat; \type)$.
\deni{I think these two comments are now answered! Seems to be a typo from before! Alec, I also added two macros into ``auxiliary/filecommands.sty'' for you to add comments make edits if you prefer that!}\amy{not sure we are maxing over the right thing here. still wondering about strategies. actually, maybe we are, but $\otherstrat$ should be $\otheraction$. and i feel like we need an expectation of types $T$.}
\alec{$\rho$ seems undefined here. Also unclear what is the difference between $\mathcal{A}$ and $\mathcal{A}^{\mathcal{T}}$ } \deni{$\actionspace$ is the joint action space, while $\actionspace^\typespace$ is the space of joint strategy profiles, i.e. mappings from typespace to action space. } \deni{Although might just need to define the strategy space because there is a problem with def'n, i.e., the current notation also includes centralized strategies.}

% \subsubsection{Contextual Games}
% A \mydef{(simultaneous-move) contextual game} \cite{sessa2020contextual} $(\numplayers, \numactions, \contexts, \initcontexts, \innerset, \typespace, \type, \reward)$ is a repeated game played over an infinite horizon which comprises of $\numplayers \in \N_+$ players each of whom is characterized by a type space $\typespace[\player] \in \subset \R^\numtypes$. At each time-step $\iter = 0, 1, \hdots$, each player $\player \in \players$ takes an action $\inner[\player][][][\iter] \in \innerset[\player](\context[\iter])$ from an action space $\innerset[\player](\context[\iter]) \subset \actionspace[\player]$\footnote{Going forward, for simplicity, without loss of generality, we drop the dependence of the action space $\innerset[\player]$ on the context $\context$ and take for all player $\player \in \players$, $\innerset[\player] \doteq \actionspace[\player]$.} simultaneously observe a \mydef{context} $\typerv[][\iter] \sim \initcontexts$, i.e., a type profile drawn from a distribution $\initcontexts \in \simplex(\typespace)$ over the set of types. Each player $\player \in \players$ , it takes an action $\inner[\player][][][\iter] \in \innerset[\player](\context[\iter])$ from an action space $\innerset[\player](\context[\iter]) \subset \actionspace[\player]$\footnote{Going forward, for simplicity, without loss of generality, we drop the dependence of the action space $\innerset[\player]$ on the context $\context$ and take for all player $\player \in \players$, $\innerset[\player] \doteq \actionspace[\player]$.}

% % Once player $\player \in \players$ has observed the realized contexts $\context[\iter]$, it takes an action $\inner[\player][][][\iter] \in \innerset[\player](\context[\iter])$ from an action space $\innerset[\player](\context[\iter]) \subset \actionspace[\player]$\footnote{Going forward, for simplicity, without loss of generality, we drop the dependence of the action space $\innerset[\player]$ on the context $\context$ and take for all player $\player \in \players$, $\innerset[\player] \doteq \actionspace[\player]$.} and receive reward $\reward[\player](\context, \inner; \type[\player])$ given by a reward function $\reward[\player]: \contexts \times \innerset \times \typespace \to \R$. For a given context, action profile, and type profile tuple, we denote the vector of all  players utilities by $(\context, \action, \type) \mapsto \reward(\context, \action; \type)$  

% A contextual game is \mydef{continuous} if for all $\context \in \contexts$, $\reward(\context, \inner; \type)$ is continuous in $\inner$ and $\innerset$ is non-empty and compact.
% A contextual game is \mydef{concave} if in addition to being continuous, for all contexts $\context \in \contexts$ and for all players $\player \in \players$, $\reward[\player](\context, \inner)$ is concave in $\inner[\player]$ and $\innerset[\player]$ is convex.

% A \mydef{(Markov or stationary) policy} \cite{maskin2001markov} for player $\player \in \players$, $\policy[\player]: \contexts \to \innerset[\player]$ is a mapping from contexts to actions such that $\policy[\player](\context) \in \innerset[\player]$ denotes the action taken by player $\player$ when it observes context $\context$. We define a \mydef{policy profile} as the collection of policies, i.e., $\policy = (\policy[1], \hdots, \policy[\numplayers]) : \contexts \to \innerset$ such that $\policy(\context) \in \innerset$ denotes the action profile played by the players under context $\context \in \contexts$. The goal of all players $\player \in \players$ is to play a policy $\policy[\player][][*] \in \innerset[\player]^\context$ which maximizes their \mydef{expected cumulative payoff} $\util[\player](\policy[\player], \policy[-\player]; \type[\player]) \doteq \Ex_{\contextrv \sim \initcontexts} \left[ \reward[\player](\contextrv, \policy[\player](\contextrv), \policy[-\player](\contextrv); \type[\player])\right]$. 
% % 


% A \mydef{$\varepsilon$-subgame perfect Nash equilibrium ($\varepsilon$-SPNE)} of a contextual game is a policy profile $\policy[][][*] \in \innerset^\contexts$ such that for all player $\player \in \players$ and for all contexts $\context \in \contexts$,  $\reward[\player](\context, \policy[][][*](\context); \type[\player]) \geq \reward[\player](\policy[\player](\context), \policy[-\player][][*](\context); \type[\player]) - \varepsilon$. A $0$-SPNE is called a \mydef{subgame perfect Nash equilibrium (SPNE)}. A SPNE is guaranteed to exist in concave contextual games. Additionally, note that when the context space is a singleton, then the SPNE of contextual game simply reduce to the NE of the game played at that context. Further, notice that the SPNE of contextual games with different context distributions are all the same.

% \sdeni{}{Overloading notation, we define the \mydef{contextual cumulative regret} at any given type profile $\type \in \typespace$, $\cumulregret[][\type]: \contexts \times \actionspace \times \actionspace \to \R$ between two action profiles $\action \in \actionspace$ and $\otheraction \in \actionspace$ across all players in context $\context$ of a contextual game as $\cumulregret[][\type](\context, \action, \otheraction) = \sum_{\player \in \players} \reward[\player](\context, (\otheraction[\player], \action[-\player]); \type[\player]) - \reward[\player](\context, \action; \type[\player])$.
% Further, the \mydef{contextual exploitability} or (Nikaido-Isoda potential function \cite{nikaido1955note}) of an action profile $\action \in \actionspace$ is defined as 
% $\exploit[][\type](\context, \action) = \max_{\otheraction \in \actionspace} \cumulregret[][\type](\context, \action, \otheraction)$ \cite{goktas2022exploit}. We note that for all $\context \in \contexts$, $\action \in \actionspace$, $\exploit[][\type](\context, \action) \geq 0$, and $\action[][][][*]$ is a SPNE of $(\numplayers, \numactions, \actionspace, \typespace, \type, \util)$ iff $\exploit[][\type](\action[][][][*]) = 0$.} 
% $\util[\player](\policy[][][*]) \geq \util[\player](\policy[\player], \policy[-\player][][*]) - \varepsilon$

% \footnote{Note that although the set of $\varepsilon$-SPNE of any contextual game $(\numplayers, \numactions, \contexts, \initcontexts, \innerset, \reward)$ is also a Nash game $(\numplayers, \numactions, \innerset^\contexts, \util)$, this reduction is mostly vacuous, as Nash's theorem \cite{nash1950existence} or Arrow-Debreu's lemma on abstract economies \cite{arrow-debreu} does not provide existence in this constructed Nash game.}
 % is a policy profile $\policy[][][*] \in \innerset^\contexts$ s.t.\ for all players $\player \in \players$ and actions $\action[\player] \in \actionspace[\player]$, $\util[\player](\action[][][][*]) \geq \util[\player](\action[\player], \action[-\player][][][*]) - \varepsilon$.
% , and for each player $\player \in \players$, an action correspondence $\innerset[\player]: \contexts \rightrightarrows \actionspace$ s.t. for any context $\context \in \contexts$ and any player $\player \in \players$, $\innerset[\player](\context) \subset \actionspace$ denotes the set of actions player $\player$ can choose under context $\context$,  who , encounter a Nash game $(\numplayers, \numactions, \innerset(\contextrv), \util())$ 

\if 0 
\deni{Decide how to incorporate this into the big story.}
\paragraph{Stackelberg-Nash Games}
An $(\numplayers + 1)$-player \mydef{Stackelberg-Nash game} $\stackgame \doteq (\numplayers, \numactions, \outerset, \innerset, \util)$ comprises one player called the \mydef{leader} and $\numplayers \in \N_{++}$ players called \mydef{followers}.
In a Stackelberg-Nash game, the leader first commits to an action $\outer \in \outerset$ from an action space $\outerset \subset \R^{\outerdim}$.
Then, having observed the leader's action, each follower $\player \in \players$, responds with an action $\inner[\player]$ in their \mydef{action space} $\innerset[\player] \subset \R^{\numactions}$.
% determined by the \mydef{feasible action correspondence} $\innerset[\player]: \outerset \rightrightarrows \actionspace[\player]$ which takes as input the leader's action $\outer$ and outputs a subset of \mydef{the action space} $\actionspace[\player] \subset \R^{\numactions}$. 
We define the \mydef{followers' joint action space} $\innerset \doteq \bigtimes_{\player \in \players} \innerset[\player]$. 
% and the \mydef{follower joint feasible action correspondence} by $\innerset(\outer) = \bigtimes_{\player \in \players} \innerset[\player](\outer) \subset \bigtimes_{\player \in \players} \actionspace[] \subset \R^{\numplayers \numactions}$
We refer to a collection of actions $\inner = (\inner[1], \hdots, \inner[\numplayers]) \in \innerset$ as a \mydef{follower action profile}, and to a collection $(\outer, \inner) \in \outerset \times \innerset$ comprising an action for the leader and a follower action profile as simply an \mydef{action profile}. 
% \deni{Maybe also define feasible action profile.} A Stackelberg-Nash game is said to have \mydef{independent action sets} if the feasible action correspondence of each player $\player \in \players$, $\innerset[\player]$ is a constant correspondence, i.e., $\innerset[\player](\outer) = \innerset[\player](\outer[][][\prime]) = \actionspace$ for all leader actions $\outer, \outer[][][\prime] \in \outerset$.

After all players choose an action, the leader receives payoff $\util[0](\outer, \inner) \in \R$, while each follower $\player \in \players$ receives payoff $\util[\player](\outer, \inner) \in \R$. 
Each player $\player \in \allplayers$ aims to maximize her payoff $\util[\player]: \outerset \times \innerset \to \R$. 
For all followers $\player \in \players$, we define the $\delta$-\mydef{best-response correspondence} $\br[\player][\delta] (\outer, \inner[-\player]) \doteq \left\{ \inner[\player] \in \innerset \mid \util[\player](\outer, \inner[][][]) \geq \max_{\inner[\player] \in \innerset[\player]} \util[\player] (\outer, (\inner[\player], \inner[-\player][][])) - \delta \right\}$ and the \mydef{joint $\delta$-best-response correspondence} $\br[][\delta](\outer, \inner) \doteq \bigtimes_{\player \in \players} \br[\player][\delta] (\outer, \inner[-\player])$. 

%\amy{we use the semi-colon notation when talking about exploitability. should we use it here as well? i tend to think yes. e.g., $\br[\player][\delta] (\inner[-\player]; \outer)$}\deni{I feel like we don't have to because this is the follower's best response in the Stackelberg game. While for exploitability that is the exploitability of the lower level game which the leader's action parametrizes so it makes sense.}

Accordingly, we define the \mydef{follower regret} $\regret[][]: \innerset \times \innerset \times \outerset \to \R^\numplayers$ for playing an action profile $\inner$ as compared to another action profile $\otherinner$ when the leader plays $\outer \in \outerset$, as follows: for all followers $\player \in \players$,
$\regret[\player][](\inner, \otherinner; \outer) = \util[\player](\outer, (\otherinner[\player], \inner[-\player])) - \util[\player](\outer, \inner)$. 
The \mydef{follower cumulative regret}, $\cumulregret: \innerset \times \innerset \times \outerset \to \R$ between two action profiles $\inner \in \innerset$ and $\otherinner \in \innerset$ across all players in a game is given by $\cumulregret(\inner, \otherinner; \outer) = \sum_{\player \in \players} \util[\player](\outer, (\otherinner[\player], \inner[-\player])) - \util[\player](\outer, \inner)$.
Further, the \mydef{follower exploitability} or (Nikaido-Isoda potential function \cite{nikaido1955note}) of a follower action profile $\inner \in \innerset$ is defined as 
$\exploit(\inner) = \max_{\otherinner \in \innerset} \cumulregret(\inner, \otherinner)$ \cite{goktas2022exploit}. 

% \if 0
% The canonical solution concept for Stackelberg-Nash games is the $(\varepsilon, \delta)$-\mydef{Stackelberg-Nash equilibrium (SNE)}, an action profile $(\outer[][][*], \inner[][][*]) \in \innerset \times \outerset$ such that:
% \begin{align}
%     \util[0](\outer[][][*], \inner[][][*]) &\geq \max_{\outer \in \outerset: \inner \in \br[][\delta](\outer, \inner)} \util[0](\outer, \inner) - \varepsilon \\
%     \util[\player](\outer[][][*], \inner[][][*]) &\geq \max_{\inner[\player] \in \innerset[\player]} \util[\player](\outer[][][*], (\inner[\player], \inner[-\player][][*])) - \delta&& \forall \player \in \players
% \end{align}
% A $(0,0)$-Stackelberg-Nash equilibrium is simply called a Stackelberg-Nash equilibrium.
% Intuitively, a $(\varepsilon, \delta)$-SNE is an action profile at which the followers play a Nash equilibrium, while the leader $\varepsilon$-approximately maximizes its payoff over its action space, assuming that the followers will play a $\varepsilon$-Nash equilibrium for any of its actions. 
% \fi


% \deni{Can remove the eqm defs, since they're in the intro.}
% \amy{not sure, b/c we don't define $\epsilon-\delta$-SE.}


As the joint best-response correspondence is not necessarily singleton-valued, the leader's objective is likewise a correspondence: i.e., multiple values could be associated with a fixed strategy $\outer \in \outerset$.
As a result, we cannot re-formulate this problem as a single objective optimization without fixing a selection criteria over the followers' joint best-responses.
The results we prove in this paper rely on the strong Stackelberg-Nash Equilibrium as a solution concept:

\begin{definition}[Strong Stackelberg-Nash Equilibrium]
A $(\varepsilon, \delta)$-\mydef{strong Stackelberg-Nash equilibrium (SSNE)} is an action profile $(\outer, \inner) \in \outerset \times \innerset$ s.t.
% 
%\begin{align}
     $\util[0](\outer[][][*], \inner[][][*]) \geq \max_{\outer \in \outerset} \max_{\inner \in \br[][\delta](\outer, \inner)} \util[0](\outer, \inner) - \varepsilon$ and
     $\util[\player](\outer[][][*], \inner[][][*]) \geq \max_{\inner[\player] \in \innerset[\player]} \util[\player](\outer[][][*], (\inner[\player], \inner[-\player][][*])) - \delta$, for all $\player \in \players$.
%\end{align}

% \begin{align}
%     \outer[][][*] &\in \argmax_{\outer \in \outerset} \max_{\inner \in \br(\outer, \inner)} \util[0](\outer, \inner)\\
%     \inner[\player][][*] &\in \argmax_{\inner[\player] \in \innerset[\player]} \util[\player](\outer[][][*], (\inner[\player], \inner[-\player][][*])) && \forall \player \in \players
% \end{align}
\end{definition}
\fi
% \begin{definition}[Weak Stackelberg Equilibrium]
% A $(\varepsilon, \delta)$-\mydef{weak Stackelberg-Nash equilibrium (WSNE)} is an action profile $(\outer, \inner) \in \outerset \times \innerset$ s.t.
% %
% %\begin{align}
%      $\util[0](\outer[][][*], \inner[][][*]) \geq \min_{\inner \in \br[][\delta](\outer, \inner)} \util[0](\outer, \inner) - \varepsilon$, for all $\outer \in \outerset$, and
%      $\util[\player](\outer[][][*], \inner[][][*]) \geq  \max_{\inner[\player] \in \innerset[\player]}\util[\player](\outer[][][*], (\inner[\player], \inner[-\player][][*])) - \delta$, for all $\player \in \players$.
% %\end{align}
% \end{definition}

%%% SPACE
% %
% \if 0
% In these definitions, the leader approximately optimizes its strategy assuming the followers approximately optimize theirs, in which case $\delta \geq 0$. \amy{i think what this means is that $\epsilon$ is a function of $\delta$.} 
% As a result, a $(0,0)$-SSNE/WSNE might not be a $(0, \delta)$-SSNE/WSNE in general.
% \deni{Can we please discuss this, I want to add a footnote but not sure how to phrase it. There is this interesting phenonmenon in the general sum-setting where computing an approximate equilibrium might be hard because the follower's approximate best-response can induce discontinuous change in the *equilibrium* strategy of the leader, and as a result a $(0,0)$-SSNE/WSNE might not be a $(0, \delta)$-SSNE/WSNE. }
% \sdeni{}{Note that an important difference above approximate Stackelberg-Nash definitions are much harder to to compute }
% \amy{i know we discussed yesterday, but need to discuss again.} \amy{i think you might want to move this discussion to right after Obs 1. it might be easier to explain there.}
% \fi

% \deni{The reason why we need the joint convexity assumption is because our goal is to compute a VE, which does not generally exist (and because projection onto non-convex sets is often hard!).}

% We also define local versions of these equilibrium concepts, which are more tractable in general. A pseudo-game is simply called a \mydef{game} if for all players $\player \in \players$, $\actions(\naction[\player])$ is a constant correspondence, i.e., for all players $\player \in \players$, and strategy profiles $\action, \otheraction \in \innerset, \actions(\naction[\player]) = \actions(\otheraction[-\player])$.


%A \mydef{local generalized Nash equilibrium (local GNE)} is an strategy profile $\inner[][][*]$ s.t.\ for all players $\player \in \players$, and $\inner[\player] \in \actions[\player](\naction[\player][][][*]) \cap \ball[\varepsilon][{\inner[\player]}]$, \amy{fix me!} $\util[\player](\inner[][][*]) \geq \util[\player](\inner[\player], \naction[\player][][][*])$.
% A \mydef{local variational equilibrium (local VE) or normalized GNE} is an strategy profile $\inner[][][*]$ s.t.\ for all strategy profiles and $\action \in \innerset \cap \ball[\varepsilon][\action]$ s.t.\ $\actionconstr(\action) \geq \zeros$, $\util[\player](\inner[][][*]) \geq \util[\player](\inner[\player], \naction[\player][][][*])$. 


% $\hypothesis \in \argmin_{\R^{\states \times \actionspace}} \nicefrac{1}{\numsamples} \sum_{\numsample \in [\numsamples]} \left\| \mathrm{Nash}\left(\hypothesis[][*](\state[\numsample]\right) - \inner[][][][\numsample]  \right\|^2$ and for all $\state \in \states$, $\hypothesis[][*](\state[\numsample])$ is a Nash equilibrium of $$.

==> conc.tex <==
\section{Conclusion}


\sdeni{}{We introduced convex-concave generative-adversarial characterization of inverse Nash equilibria for a large class of games, including normal-form, finite state and action Markov games, and a number of continuous state and action Markov games. This novel formulation then allowed us to obtain polynomial-time computation guarantees for inverse equilibria in these games, a rather surprising result since the computation of a Nash equilibrium is in general PPAD-complete. Our result can be thus seen as a positive computation result for game theory. We then extended our characterization to a multiagent apprenticeship learning setting, where we souught to not only rationalize the observed behavior as an inverse Nash equilibrium but also make predictions based off the inverse Nash equilibrium, and have shown in experiments on prices in Spanish electricity markets that our approach to solving multiagent apprenticship learning can be effective at predicting behavior in multiagent systems. The approach to inverse game theory that we provided in this paper is a highly flexible one and thus can be used to solve inverse equilibrium beyond inverse Nash equilibria and future work could explore ways to extend our approach to other game-theoretic settings and equilibrium concepts.}


\amy{discuss extenstion to other eqm concepts? CE, CCE, etc.}

\amy{and other idea from yesterday. check text thread?}




==> counterfactual_pred.tex <==
\section{Strategic Counterfactual Prediction \deni{Name subject to change, but I like it rn}}
% \deni{Make everything in terms of the distribution!!!}

% \deni{Realizable case first, and then unrealizable case? I think so.}
\deni{Not in love with notation.}
Consider a supervised learning problem $(\contexts, \contextdistrib, \outcomes, \{\context[\numsample]\}_{\numsample \in [\numsamples]}, \{ \optsol(\context[\numsample])\}_{\numsample \in [\numsamples]}, \hypotheses) $ which consists respectively of some \mydef{contexts} and associated \mydef{outcomes} $ \{\left( \context[\numsample], \outcome[][\numsample] \right)\}_{\numsample \in [\numsamples]} \sim \contextdistrib^\numsamples$ drawn from some distribution $\contextdistrib \sim \simplex(\contexts \times \outcomes)$ over a \mydef{context space} $\contexts$ and \mydef{outcome space} $\outcomes$.  \deni{Might call this an outcome statistic, or something along those lines.} 
% $\{ \outcome[][\numsample] \}_{\numsample \in [\numsamples]} \subset \outcomes$ coming from an 
Our goal is to learn a \mydef{hypothesis} $\outcomemap[][*]: \contexts \to \outcomes$, a mapping from the context space to the outcome space, in the \mydef{hypothesis space} $\outcomemap \subset \outcomes^\contexts$ that replicates the marginal distribution over outcomes most closely, e.g., taking the euclidean distance as a distance metric find $\outcomemap[][*] \in \argmin_{\outcomemap \in \outcomemaps} \Ex_{(\contextrv, \outcomerv) \sim \contextdistrib} \left[ \left\| \outcomerv - \outcomemap(\contextrv)\right\|^2 \right]$. 
The standard approach to learn such a mapping is to find a hypothesis in the hypothesis class that minimizes the \mydef{empirical error}, i.e.,  $\outcomemap[][*] \in \argmin_{\outcomemap \in \outcomemaps} \left[ \nicefrac{1}{\numsamples} \sum_{\numsample \in [\numsamples]} \left\| \outcome[][\numsample] - \outcomemap (\context[\numsample]) \right\|^2 \right]$. Although one can choose $\outcomemaps$ to be any hypothesis class, such an approach might prove to be inefficient for certain problems. For instance, if the optimal hypothesis is not a Lipschitz-continuous function, then the sample complexity of learning the optimal hypothesis can be exponential in the worst case, i.e., require an unacquirable amount of data which would be intractable to process. An example of such problems is the class of strategic counterfactual prediction problems. \deni{probably a majority of this discussion will have to be moved to the intro.} 

In strategic counterfactual prediction problems, we seek to predict the outcome of the interaction of rational agents if a different state of the world were to occur. For instance, consider first price auctions for a set of varying goods and a set of fixed bidders. Given access to a history of contexts, e.g., goods auctioned, and outcomes, e.g., the highest winning bids, we are often interested in predicting the \sdeni{winner}{winning bid} \amy{actually, we are usually interested in predicting the price, not the winner; i.e., something continuous, not discrete} \deni{I think the edit fixes the concern?} of an auction for a different set of goods, i.e., the state of the world, for the same bidders. As an auction can be modelled as a Bayesian game, for predictions in such problems to be good, it is often necessary to ensure that the predictor that is learned also captures the underlying Bayesian game model of the auction. That is, by fitting a Bayesian game to the contexts, i.e., learn a mapping from contexts to types such that the EPNE of the associated game replicates the history of highest winning bids most accurately. Unfortunately, learning such a model over a very broad hypothesis class $\hypotheses$ is often not feasible since Nash equilibria are not in general continuous in their parameters,  and as such, learning such a mapping using traditional function approximation methods, e.g., training a feedforward neural network, will often overfit to the data and not lead to learning a game theoretic model due to the possibly exponential sample complexity of the problem for general hypothesis classes. 


\deni{Need a description of the game here first.} However, if we choose to fit a game-theoretic model to the data a priori and specify a game structure $(\numplayers, \numactions,  \typespace, \actionspace, \util)$, consisting of a number of players $\numplayers \in \N_{++}$, an action space dimension $\numactions \in \N_{++}$, a joint type space $\typespace \doteq \bigtimes_{\player \in \players} \typespace[\player] \subset \R^{\numplayers \times \numtypes}$, a joint action space $\actionspace \doteq \bigtimes_{\player \in \players} \actionspace[\player] \subset \R^{\numplayers \times \numactions}$, and a payoff structure $\util: \actionspace \times \typespace \to \R^\numplayers$, we can restrict our hypothesis class to functions from contexts to outcomes which are compositions $\outcomemap \circ \eqmmap \circ \typemap$ of (a) a \mydef{type mapping}, i.e., mappings $\typemap \in \typemaps \doteq \{ \typemap: \contexts \to \typespace \}$ from contexts to types, (b) an \mydef{equilibrium mapping}, i.e., mappings $\eqmmap \in \eqmmaps \doteq \{ \eqmmap: \typespace \to \actionspace\}$ from types to (possible approximate equilibria and (c) an \mydef{outcome mapping}, i.e.,  mappings $\outcomemap \in \outcomemaps \doteq \{\outcomemap: \actionspace \to \outcomes\}$ from equilibria to outcomes. This restriction can in turn significantly reduce the domain of our search and can as such overcome issues of sample complexity and overfitting. Unfortunately, techniques to learn such mappings from data few and far between, and often work for limited classes of games or simplistic solution concepts or make very strong assumptions, e.g., uniqueness of equilibria. This dearth of literature, points to a need to develop methods that can fit games to data regardless of the type of the game. \deni{Need more discussion on PPAD-completeness and yaddeyyaddah.}

With \Cref{obs:bne} now in hand, we can however provide a mathematical characterization of mappings $(\outcomemap, \eqmmap, \typemap) \in \outcomemaps \times \eqmmaps \times \typemaps$ such that the hypothesis $\outcomemap \circ \eqmmap \circ \typemap$ minimizes the supervised learning loss, while the mapping $\eqmmap$ is a $\varepsilon$-EPNE.\footnote{Once again, in this work we focus on EPNE but we note that our results also apply to the more general solution concept of the BNE.} 
\begin{align}\label{eq:GGS}
    & \min_{(\typemap, \eqmmap, \outcomemap) \in \typemaps \times \eqmmaps \times \outcomemaps} & \nicefrac{1}{\numsamples} \sum_{\numsample \in [\numsamples]} \left[\left\|\outcomemap(\eqmmap(\typemap(\context[\numsample]))) - \outcome \right\|^2 \right]\\
    &\text{Subject to } &  \nicefrac{1}{\numsamples} \sum_{\numsample \in [\numsamples]} \exploit[][](\eqmmap(\typemap(\context[\numsample])); \typemap(\context[\numsample])) \leq \varepsilon
\end{align}
The above problem can be interpreted as a two-player general-sum game between a generator who chooses mappings $(\typemap, \outcomemap) \in \typemaps \times \outcomemaps$ from contexts to types and action profiles to outcomes, and a simulator who chooses a mapping $\eqmmap \in \eqmmaps$ from types to action profiles. The goal of the generator is to pick mappings which result in a game who equilibria replicate the outcome data most accurately, while the goal of the simulator is to simulate the EPNE associated with the game. 
The optimal mappings $(\outcomemap[][*], \eqmmap[][*], \typemap[][*]) \in \outcomemaps \times \eqmmaps \times \typemaps$ that solve \Cref{eq:GGS} are then called the \mydef{generative game simulator}. 


% To address this need, we introduce the \mydef{generative game simulator} which consists of finding a predictor $\hypothesis[][*]$ which maps each context to a type, and computes for this type a (possibly approximate) Nash equilibrium and outputs a function of this Nash equilibrium. More precisely, given $(\numplayers, \numactions,  \typespace, \actionspace, \util)$ consisting of specification of a Bayesian game where the type distribution and type distribution parameter  is unknown, the counterfactual learning consists of solving the following problem:
% \deni{EPNE in a Bayesian game}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.25]{figures/summary figure.jpeg}
%     \caption{Summary of the Counterfactual Prediction Framework}
%     \label{fig:summary}
% \end{figure}



% Consider a prediction problem $(\contexts, \contextdistrib, \outcomes, \{\context[\numsample]\}_{\numsample \in [\numsamples]}, \{\outcome[][\numsample] \}_{\numsample \in [\numsamples]}) $ which consists respectively of some \mydef{contexts} $\{\context[\numsample]\}_{\numsample \in [\numsamples]} \sim \contextdistrib^\numsamples$ drawn from some distribution $\contextdistrib \sim \simplex(\contexts)$ over a context space $\contexts$ and some associated \mydef{outcomes} $\{ \outcome[][\numsample] \}_{\numsample \in [\numsamples]}$  outcome space $\outcomes$. Our goal is to learn a \mydef{predictor} $\hypothesis: \contexts \to \outcomes$ from the context space to the outcome space that most closely replicates the joint distribution over the context and outcome space when given the access the marginal distribution over the context space

==> figure.tex <==
% \begin{figure}
% \centering
% \begin{subfigure}{.45\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figures/gen_adv_exact_summary.png}
%   \caption{Generative-Adversarial Inverse Game Theory \amy{maybe the figure should say $x_i \in \mathcal{X}(x^*_{-i})$, under Best Responses}}
%   \label{fig:sub1}
% \end{subfigure}%
% \quad \vline \quad
% \begin{subfigure}{.45\textwidth}
%   \centering
%   \includegraphics[width=1\linewidth]{figures/gen_adv_stoch_summary.png}
%   \caption{A subfigure \amy{i'm unclear about this best responses. should the eqm generated be $x^*$? and then same comment here as in figure (a)? or maybe use $\hat{x}$ instead of $x^*$, since we are less sure this $x$ is an eqm.}}
%   \label{fig:sub2}
% \end{subfigure}
% \caption{Generative-Adversarial Inverse Multiagent Learning}
% \label{fig:test}
% \end{figure}


% \begin{figure}
%   \centering
%   \subfigure[Subfigure 1]{
%     \includegraphics[width=0.5\textwidth]{figures/gen_adv_exact_summary.png}
%   }\label{fig:gen_sim_fig}
%   \subfigure[Subfigure 2]{
%     \includegraphics[width=0.5\textwidth]{figures/gen_adv_stoch_summary.png}
%   }
%   \caption{Two subfigures side by side.}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[scale=0.3]{figures/gen_adv_exact_summary.png}
%     \caption{\deni{FIGURE HAS TO BE UPDATED, WE ARE IN A GENERAL SUM WORLD NOW!}A summary of the Generative Game Simulator}
    
% \end{figure}


==> intro_OLD.tex <==
\section{Introduction}

%\amy{i am not sure if we want to say stochastic or noisy oracle? we also have lossy and lossless.}

\amy{
\begin{itemize}
\item
\end{itemize}
}

Game theory is a mathematical framework used to predict the outcome of the interactions, called games, of preference-maximizing agents, called players, whose preferences among outcomes are represented via payoff functions.
%%% SPACE
%\footnote{While it is commonly assumed \amy{what do you mean assumed? vN\&M PROVED a theorem saying that this is so!}\deni{This is me making a point against an argument which I see people utter all the time and I hate. People say that game theory is doomed because everything assumes rationality, i.e., payoff maximizing behavior. This is wrong. The paper I cite at the end of this footnote proves the existence of a \samy{Nash}{Walrasian} equilibrium for preferences which CANNOT be represented as payoff maximization problems. In fact, they make so few assumptions on the preference relation that they show that even ``irrational'' preferences \samy{outcome can be modelled as NE}{can lead to equilibrium behavior}.} that players' preferences can be represented via payoff functions under suitable assumptions on the preferences (i.e., completeness and transitivity), game theory and its predictions \samy{}{also} concern the interaction of agents whose preferences might not be representable via payoff functions \citep{mas1974equilibrium, shafer1975equilibrium}. \amy{this paper is actually about Walrasian eqm, not Nash. so are you assuming a reduction from one to the other?} \deni{Ah it seems I was missing on references, Shafer's paper generalizes the result to pseudo-games.}}
The canonical outcome, or solution concept, prescribed by game theory is the equilibrium: an action profile, i.e., a collection of actions, one per player, such that each player's action is rational, i.e., payoff maximizing, contingent on the payoff-maximizing behavior of the others.
When using game theory to make a prediction, it is typical to assume that \samy{the model of players' behavior, including their preferences, is}{the players' preferences are} known. 
%\amy{the behavioral model includes more than the preferences. it also includes whether they are rational, boundedly rational, etc. so maybe you mean e.g., instead of i.e., right after this comment:}\deni{Imo, a preference relation can represent any behavior, including boundedly rational behavior as long as we make no assumptions on the preference relation? but I will make the change} 
However, in many applications of interest, such as contract design \citep{holmstrom1979moral, grossman1992analysis} and
counterfactual prediction \citep{peysakhovich2019robust}, 
%and apprenticeship learning \citep{donge2022multi}, 
\samy{a behavioral model}{complete preference information} is not available; only the choices the players make are observable.
In such cases, we may seek to identify payoff functions\samy{}{---from a space of parameterized payoff functions---}that replicate the observed actions.
Assuming these actions are equilibrium actions, this identification task serves to \mydef{rationalize} them.
Identification problems of this nature characterize \mydef{inverse game theory} \citep{waugh2013computational, bestick2013inverse}.

The object of study of inverse game theory is the \mydef{inverse game}, which comprises a set of players, each characterized by an action space and a parametric payoff function \samy{}{with relevant parameters omitted},
%mapping the players' actions to a real number,
replaced by an observed 
%\amy{possibly mixed? or realized samples?} 
action profile. 
%\amy{we are also given a behavioral model in an inverse GT problem}
Given an inverse game, the goal is to compute an \mydef{inverse equilibrium}, i.e., parameter values such that the observed actions correspond to an equilibrium
%\samy{}{, under the given behavioral model,} 
of the payoff functions evaluated at those values.
\samy{}{Our first contribution is to formally pose and solve this problem, assuming access to an \emph{exact\/} oracle that returns the payoffs of queried action profiles.}
%\deni{Ok I think now this matches with the rest of the text and makes a lot of sense, thanks!!} \amy{well, i still don't like it!}
%As deterministic equilibria are not guaranteed to exist, players' actions and thus their payoffs can be stochastic, in which case the latter cannot be accessed directly and instead have to be estimated via simulation.\amy{REWRITE!}
%
Relaxing the assumption of an exact oracle, and instead assuming access to a game simulator that can be used to estimate the players' payoffs (i.e., a \emph{stochastic\/} oracle), brings us from the realm of inverse game theory into the realm of \mydef{inverse multiagent learning}.
%\sdeni{}{More generally, when the game is also non-stationary \amy{i really do not get this claim about non-stationarity. Markov games are stationary!!! maybe NE policies are not in general, but the themselves games are.}, the relevant model is that of stochastic (or Markov) games \citep{shapley1953stochastic,takahashi1964equilibrium,fink1964equilibrium}---time-based games where players observe a new state at each time-step and simultaneously take actions which stochastically determines their next state and yields an instantaneous payoff---}
When the underlying game is also stochastic, the relevant problem is one of \mydef{inverse multiagent reinforcement learning} (inverse MARL) \citep{russell1998learning, ng2000algorithms,natarajan2010multi}.
\samy{}{Our second contribution is to solve inverse MARL.
We solve both inverse game theory and inverse MARL in the \emph{online\/} case, where we assume simulator access and can thus sample any trajectory of play associated with an observed equilibrium.}

%\amy{does Ng really attempt inverse MARL in that first 2000 paper? i didn't remember that?} \deni{No the first two papers are pure IRL but felt appropriate to cite, we can remove tho.}
%One can similarly define various equilibrium concepts such as Nash equilibrium for stochastic games, but now in terms of policy profiles (i.e., mappings from states to action profiles), and then seek to compute game parameters (i.e., an inverse equilibrium) that rationalize observed behavior.
%\amy{how is it an instance of inverse MARL if we no longer have a simulator/generative model? isn't then apprenticeship learning the more general problem?} is 

More generally, in
\mydef{multiagent apprenticeship learning} \citep{abbeel2004apprenticeship, yang2020inferring}, the goal is to find a policy profile that rationalizes the players' observed behavior, given sample trajectories of play prepared \emph{offline}.
We study a yet more general version of this problem in which the observations are mere summaries of sampled agent behaviors, rather than the samples themselves, e.g., an aggregate demand curve for an economy, rather than all the individuals' demands.
This generalization of multiagent apprenticeship learning involves finding a \mydef{simulacrum}, meaning parameter values together with associated equilibrium policies that replicate the observed trajectories of play as samples from the simulacrum policies, in expectation.
\samy{}{By solving this 
%``simulacrum learning'' 
problem, we not only provide an explanation of the agents' observed (offline) behavior, which, upon computing an ensuing equilibrium, can be used to predict their future behavior, should the state of the world remain constant; we further provide counterfactual predictions of unobserved behavior, should the state of the world change.}

\amy{i guess it makes some sense to call the more general problems we are defining: simulacrum planning and learning.}

%Given noisy payoff samples obtained by simulating the players' policies,\amy{this sounds just like inverse MARL; distinction is not clear}\deni{I think if you are referring to the idea of learning only from samples, I think that's a step ahead, and would be offline multiagent apprenticeship learning, which is a contribution we make but I think it should be part of the contributions.}

\if 0
in the \mydef{online} case, where we assume simulator access and can thus sample any history associated with an observed equilibrium.
in the \mydef{offline} case, where we have only a noisy sample of realized equilibrium histories. 
%associated with an unobserved equilibrium.
\amy{histories or trajectories? be consistent!}
\fi

% \sdeni{}{in expectation replicate} an observed sample trajectory drawn from this policy profile as an equilibrium. 
% \amy{DEFINE SIMULACRUM here! talk about what replication means: i.e., only in expectation!}

% \amy{probably delete:} \samy{However, due to the non-stationarity of the game as well as possible stochasticity of the policies, one often cannot observe the entire policy, but rather only noisy samples of (state, action) tuples, and has to learn parameters from these samples.}{} 
%For instance, if we seek to model and explain the movement of two teams of soccer players on the field, we might at any second observe the positions of the players on the field, but we will never observe their movement in every single possible positioning of the player on the field.\amy{i'm not convinced. with cameras overhead, we can observe everyone's movements. i think you mean to say that we do not observe their policies. but you have not said this.}


\deni{Mention that we will focus on Nash equilibrium.}
\amy{this paragraph doesn't fit here. move to conclusion, perhaps. as future (mostly empirical) work!}
\amy{and if this paper at present has no conclusion, write one, or just delete this paragraph for now. don't worry---i know how it pains you do this, since you you LOVE my 2003 paper so much! :) but copy to conc.tex file, so we don't forget about it!} \deni{it really is a brilliant paper, idk why it's not your most cited one!!!} \amy{easy answer. b/c the correlated-Q paper, which is actually a source of great embarrassment to me, was picked up by DeepMind people! and therefore, it is highly cited. sigh!}
Common solution concepts for inverse game theory problems are \mydef{Nash}, \mydef{correlated}, and \mydef{coarse correlated equilibrium}, in which case we refer to the associated inverse equilibrium concepts as inverse Nash, inverse correlated, and inverse coarse correlated equilibrium, respectively.
At these and all equilibria, the players' feel no \mydef{regret} for not having played some other action, given the actions of the others.
The available \mydef{counterfactual deviations} (i.e., alternative behaviors), which generate these regrets, define the various equilibrium concepts.
In this paper, we focus on the inverse Nash equilibrium problem, but our characterization and algorithms can easily be extended to other inverse equilibrium concepts, and to inverse equilibrium problems beyond games \citep{arrow-debreu, facchinei2010generalized}).
%\amy{to pseudo-games}


A growing literature has been dedicated to the inverse game theory and inverse multiagent reinforcement learning problems under various guises, including parameter identification in econometrics \citep{wright1928tariff, syrgkanis2017inference}, model estimation in microeconomics/macroeconomics \citep{taylor1979estimation}, and multiagent immitation learning \citep{song2018multi}.
While some progress has been made in providing a mathematical characterization of inverse correlated equilibrium in normal-form games \citep{waugh2013computational, kuleshov2015inverse, syrgkanis2017inference} and inverse Nash equilibrium in restricted classes of finite state and action  games \citep{lin2017multiagent, lin2019multi}, very little is known about the computational complexity of inverse Nash equilibrium in normal-form or general-sum  games.
Furthermore, most theoretical guarantees for algorithms that compute inverse equilibria concern inverse correlated equilibria in inverse normal-form or Bayesian games with discrete actions; very little is understood about the computational complexity of inverse Nash equilibria in general-sum normal-form or  games, the latter with continuous action or state spaces.
%\sdeni{, or the sample complexity of the inverse equilibria in stochastic games, where only sample trajectories from equilibrium policies may be observed}{}.\amy{i am not sure if this second half of the sentence is supposed be crossed out or not.} \deni{Supposed to be crossed-out.}
This paper aims to develop a flexible mathematical and algorithmic framework to solve inverse equilibrium problems efficiently in a wide variety of games for various choices of equilibrium concepts, with the ultimate goal of making counterfactual predictions based on \samy{inverse}{observed} equilibria.

\amy{but we assume an observation distribution --- which is a form of a simulator. weaker than simulating policies and observing rewards. but we do simulate policies and observe ``observations'', which are functions of/lossy rewards.}

\alec{there are a lot of terms being thrown around...would it be possible to visualize a schematic of the inverse MARL/equilibrium computation problem? i.e. given time-series of, e.g. prices, rationalizing the demand is associated with computing some equilibrium? Perhaps a little cartoon of what it looks like for energy market or congestion game? specifically a diagram could depict what the generator and discriminator does in the inverse multi-agent game setting}

\alec{another comment is that I don't think we defined normal-form or general-sum anywhere. What does it mean with respect to agents' utility functions/how they interact?}
%\amy{Alec, please create and use a macro. o/w, we cannot automatically turn off your comments to submit!}

We formulate the problem of computing an inverse equilibrium \sdeni{}{(resp.\@ simulacrum)} in inverse games as a generative adversarial optimization problem between a generator and a discriminator.
The generator takes as input the observed action/policy profile \sdeni{}{(resp.\@ observed trajectories)}, based on which it generates candidate parameter values \sdeni{}{(resp.\@ parameter values and associated equilibrium policies)} for the players' parametric payoff functions, which the discriminator then judges by computing possible unilateral utility-improving counterfactual deviations.\amy{not the typical use of discriminator!}
%at the generator's parameters. 
In computing inverse equilibria (resp.\@ simulacra), the generator's goal is to choose parameters (resp.\@ parameters and a candidate equilibrium) that minimize the cumulative regret across all players
%(i.e., the sum of the per-player changes in utility for unilaterally deviating from one profile to another)
between the observed (resp.\@ candidate) equilibrium and the profile chosen by the discriminator, while the goal of the discriminator is to choose a profile that maximizes this regret.\amy{not the typical use of discriminator!}
Our formulation is fully general in the sense that it can be extended to any game and equilibrium concept for which a notion of regret is well-defined (see, for instance \citep{morrill2022hindsight}).

Our methods provide an efficient way to fit game-theoretic models onto real-world data, and in the case of multiagent apprenticeship learning, make behavioral predictions. 
To demonstrate this fact, we model the Spanish electricity market as a game between electricity re-sellers who set prices so as to maximize their profit and consumers who demand electricity so as to maximize their utilities.
We then compute a Nash simulacrum that replicates real-world price and demand in this market through 2018, which we test on electricity prices from 2018 to 2020 by simulating the simulacrum policies.

%\sdeni{}{Finally, we show that our formulation can be extended to multiagent apprenticeship learning, where the goal is not only to explain observed behavior but to also replicate it.}

% then takes as input based on which it outputs an equilibrium for the game associated with these payoff functions.
% Our method is ``generative,'' as it generates parameters of a game, that are intended to reproduce equilibria; and it is ``simulative'' as it can only simulate the equilibrium associated with the generated parameter.
% GGS can be used to compute an inverse equilibrium whenever the exploitability, i.e., distance of an action profile from an equilibrium in payoff space, can be computed efficiently.  


% \amy{all this stuff about the Spanish electricity market belongs somewhere in the introduction.}
% For instance, in our experimental set-up in \deni{Add spanish electricity  market prices experiement forward ref.}, we model the Spanish electricity market as a game between electricity re-sellers who set prices so as to maximize their profit and consumers who demand electricity so as to maximize their utilities.
% In this setting, electricity providers only collect data on prices and the aggregate demand of the consumers, not the particular demands of the individual consumers, which comprise their equilibrium actions.
% %, the sum of the demands across all consumers. 
% As such, we do not have access to individual electricity consumptions, meaning that in our game model the observation distribution takes as input price and demand policies of the sellers and consumers respectively and outputs a trajectory of prices for the sellers, and \emph{the sum} of the demand trajectories across all consumers.  


==> inverse_contextual.tex <==
% \section{Counterfactual Prediction and Contextual Games}
\subsection{Inverse Markov-Nash Equilibrium}

While a large body of work has been devoted to the computation of inverse $\varepsilon$-NE (see \deni{add backward references to related works section.}), the inverse $\varepsilon$-NE has limited use in making counterfactual predictions since \deni{non-uniqueness, ... why??}. \deni{Insert: More references and broader discussion.} 
A more interesting game-theoretic model of counterfactual prediction is instead that of the contextual inverse $\varepsilon$-Nash equilibrium problem.

An \mydef{inverse Markov game} $(\numplayers, \states, \actions, \params, \reward, \trans, \discount, \initstates, \policy[][][*])$ consists of $\numplayers \in \N_+$ players who have played a policy profile $\policy[][][*]$ in a Markov game $(\numplayers, \states, \actions, \params, \param^*, \reward, \trans, \discount, \initstates)$ where the parameter $\param \in \params$ has not been observed.
% , i.e., the parameter $\param \in \params$ defining the common type prior $\typedistrib[\param] \in \simplex(\typespace)$ is unknown
Our goal is to recover the game parameter assuming that the players played a (possibly approximate) NE (resp. MPNE). That is, we seek to compute a \mydef{$\varepsilon$-inverse NE} (resp \mydef{$\varepsilon$-inverse MPNE)}, a parameter $\param^* \in \params$ over types such that $\strat[][][*]$ is a $\varepsilon$-BNE of $(\numplayers, \numactions,  \typespace, \typedistrib, \param^*, \actionspace, \util)$
% \footnote{In this work, we focus on the EPNE, a refinement of BNE, but we note that the following observation applies more generally to BNE as well by simply pulling the maximum in the constraint outside of the expectation.}
.
% with each player $\player \in \players$ having an \mydef{action space} $\innerset[\player] \subset \R^{\numactions}$, a \mydef{type space} $\typespace[\player] \subset \R^\numtypes$, and parametric type-dependent form over payoff functions \cite{}. We denote the joint action and type spaces respectively by $\innerset \doteq \bigtimes_{\player \in \players} \innerset[\player]$ and $\typespace \doteq \bigtimes_{\player \in \players} \typespace[\player]$. The game is characterized by a context distribution $\initcontexts \sim \simplex(\contexts)$ over contexts $\contexts \in \R^\numcontexts$ and over the payoff function. 
% The players have played a $\varepsilon$-SPNE $\strat[][][*] \in \actionspace$ in the contextual game but we unfortunately have not observed the players' types and have only knowledge of function form payoff functions, i.e., $\utilspace \subset  \{\left(\util[\player]: \actionspace \times \typespace[\player] \to \R\right)_{\player \in \players} \}$.
% The solution to an inverse game is the 

% consists of finding an \mydef{inverse equilibrium mapping} $\hypothesis[][*]: \states \to \R^\actionspace$, which takes takes as input a state $\state \in \states$ and outputs utility functions $\hypothesis[][*]\left[\state\right]: \actionspace \to \R^\numplayers$ s.t. for all samples $\numsample \in \numsamples$, $\hypothesis[][*](\state[\numsample])$ $\varepsilon$-rationalize $\inner[][][*][\numsample]$. 


\deni{HAVE TO FIX EPNE exploitability.}

\amy{assume players play eqm in expection wrt some distribution, goal is to rover this distribution from observed play}


\begin{observation}\label{obs:bne}
    Suppose that the set of inverse EPNE of  $(\numplayers, \numactions, \typespace, \typedistrib, \actionspace, \util, \strat[][][*])$ is non-empty. Then, the set of types which solve the following (bi-level) optimization problem is equal to the set of inverse EPNE of $(\numplayers, \numactions, \contexts, \innerset, \initcontexts, \util, \typespace, \typedistrib, \strat[][][*])$:
    \begin{align}
        & \min_{\substack{\param \in \params \\ \policy \in \actionspace^\states}} &\left\|\policy[][][*] - \policy \right\|^2\\
        &\text{subject to } & \max_{\otherpolicy \in \actionspace^\states} \cumulregret[][](\policy, \otherpolicy; \param) \leq 0
    \end{align}
\end{observation}

\begin{proof}
    \deni{Modify proof here: }

     Let $(\type[][][\mathrm{OPT}], \action[][][][\mathrm{OPT}])$ be the optimal solutions to the above optimization problem. Then, note that by the constraint, we have:
    \begin{align}
         \exploit[][{\type[][][\mathrm{OPT}]}](\action[][][][\mathrm{OPT}]) =  \max_{\otheraction \in \actionspace}\cumulregret[][{\type[][][\mathrm{OPT}]}](\action[][][][\mathrm{OPT}], \otheraction) \leq \varepsilon
    \end{align}
    Hence, $\action[][][][\mathrm{OPT}]$ is a $\varepsilon$-NE. Now suppose that $\action[][][][\mathrm{OPT}] \neq \action[][][][*]$, then we could find a utility function for which $\action[][][][*]$ is the $\varepsilon$-NE since the set of inverse $\varepsilon$-NE is non-empty, and decrease the objective value, a contradiction.
\end{proof}

\begin{remark}
    Similar to \Cref{obs:inverse_NE}, the above observation tells us that inverse BNE problem 
\end{remark}

\begin{theorem}[Convergence proof]
    
\end{theorem}

\begin{theorem}[Sample Complexity]
    
\end{theorem}
% \deni{Add second observation over here:}
% We now introduce a Stackelberg-Nash game formulation of the inverse Nash equilibrium problem.

% \begin{align}
%     \min_{\hypothesis } \min_{\inner} \left\| \inner(\state[\numsample]) - \inner[][][*][\numsample]  \right\|^2\\
%     \text{s.t.} \sum_{\numsample \in \numsamples} \exploit(\inner(\state[\numsample]);\hypothesis(\state[\numsample])) \leq 0 
% \end{align}


% \sdeni{}{, but can be indirectly accessed via a context $\contextrv \doteq \f(\typerv)$ where $\f: \typespace \to \contexts$ is a mapping from types to contexts. We denote the context distribution  $\contextdistrib \sim \simplex(\contexts)$}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> notes.tex <==
\section{Intro Outline}

\amy{
\begin{itemize}
\item introduce game theory, including eqm definition. need to discuss how general this def'n should be. 
%
\begin{itemize}
\item do we really need CF deviations this early? might be too specific/detailed for first paragraph.
%
\item otoh, we could introduce parameterized-payoff this early, since they are fundamental to our story
\end{itemize}
%
\item define inverse game theory: payoffs are unknown. (again prob don't need to worry about Nash vs. CE vs. CCE, etc.)
%
\item four versions of the problem are known/have been studied: planning vs.\ learning, depending on whether oracle is exact or stochastic. and inverse vs. apprenticeship (planning or learning), depending on whether exact policies are known, or only samples from those policies are given.
%
\item we consider a further breakdown of the apprenticeship learning problem in particular. in the usual version, the samples are fine-grained. we also consider a more realistic version, in which the samples are coarser. while the solution to the former problem is an equilibrium, we call the solution to this latter problem a *simulacrum*. we call the problem itself, high-fidelity inverse MARL (MAYBE!!!/placeholder).
%
\item first contribution: solve inverse game, given eqm policies, assuming an exact oracle. Inverse MAP. 
%
\item second contribution: solve inverse game, given eqm policies, assuming stochastic oracle. Inverse MAL. actual application is to stochastic games, so we solve Inverse MARL.
%
\item third contribution: solve inverse game, given sample trajectories of eqm policies, assuming stochastic oracle. this problem is called multiagent apprenticeship learning. in fact, we solve a generalization of multiagent apprenticeship learning, namely ???, in which the sample trajectories are COARSE-grained/low-resolution.
%
\item N.B. i remain uncomfortable equating behavioral models and payoffs...still thinking about this point. (and wrote to a behavioral economist to inquire.)\deni{We should not use the term behavioral model anywhere. I removed any mention. It is not necessary for what we are doing.}
\end{itemize}
}


\section{Notes}

% \begin{enumerate}
%     % \item Was the GAES method computing a Bayesian coarse correlated equilibrium \deni{There seems to be a bug in the def'n of CCE for Bayesian games, need to ask Gianluca or someone else.}
%     % \item Relation between Bayesian coarse correlated equilibrium and Nash eqm.?
%     % \item Auction example
%     % \item Major difference between Vasilis' paper and this is that Vasilis works in a discretized setting.
%     % \begin{enumerate}
%     %     \item In particular: Correlated in continuous action space does not make sense, instead one would be better off considering Nash in mixed strategies which would be better and as easy to solve. The whole thing does not make too much sense.
%     % \end{enumerate}
% \end{enumerate}

==> related_old.tex <==
\paragraph{Related Work}

\paragraph{Min-max optimization}
When $\obj = -\otherobj$, a bilevel optimization problem reduces to a min-max optimization problem, or a zero-sum Stackelberg game. \sdeni{}{A variety of algorithm have been developed to solve such games in recent years (for a summary, see for instance, \cite{lin2020near, lin2020gradient}).}
Such games have also found many applications in machine learning, including but not limited to generative adversarial networks (GANs) \cite{goodfellow2014gan}, statistical learning \cite{xu2009robustness, shafieezadeh2015distributionally, dai2019kernel}, online learning \cite{cesa2006prediction}, deep learning \cite{sinha2017certifiable, sinha2020certifying}, distributed computing \cite{shamma2008cooperative, mateos2010distributed}, fairness in machine learning \cite{dai2019kernel, edwards2016censoring, madras2018learning, sattigeri2018fairness, xu2018fairgan}, and generative adversarial imitation learning \cite{cai2019global, hamedani2018iteration}.


\paragraph{Bilevel Optimization.} 
Many algorithms to solve bilevel optimization problems have been introduced in recent years.
\citeauthor{ghadimi2018approximation} (\citeyear{ghadimi2018approximation}) proposed a nested gradient descent ascent, which they call the bilevel approximation method, and which converges to a Stackelberg equilibrium in $O(\nicefrac{1}{\varepsilon})$ under the assumption that the leader's payoff is concave and the followers' payoff is strongly concave and unconstrained.
Under similar assumptions \citeauthor{ji2021bilevel} (\citeyear{ji2021bilevel}) proved tighter convergence bounds,
%to a Stackelberg equilibrium for the nested gradient descent ascent method, 
while \citeauthor{yang2021achieving} (\citeyear{yang2021achieving}) derived an
%nested gradient descent ascent 
algorithm that converges \amy{similar convergence guarantees?} 
%to a Stackelberg equilibrium
in a decentralized setting.
\citeauthor{hong2020two} (\citeyear{hong2020two}) subsequently provided a two time-scale algorithm, which consists of only a single gradient descent ascent loop, and which converges \amy{same rate?} under the same assumptions.\amy{which assumptions? also decentralized?}
\citeauthor{chen2021closing} (\citeyear{chen2021closing}) provided a tighter analysis of this latter algorithm, albeit under the assumption that the leader and followers' problems are unconstrained.
\citeauthor{chen2021closing} (\citeyear{chen2021closing})'s method improves upon previous work by using an additive correction term in the follower update step (beyond a basic SGD step).\amy{wait, is this the correct reference? the previous sentence said they analyze the same algo? not that they introduce a new method?}

There also exists a parallel line of work within game theory, which has focused on computing variants of Stackelberg equilibrium in single-leader-single-follower Stackelberg games.
These works include methods to compute first-order Stackelberg equilibria in games where the best-response of the follower is \amy{not?} unique \cite{fiez2019convergence, fiez2020implicit}, strong Stackelberg equilibria in Stackelberg games with discrete-action spaces, i.e., Stackelberg security games \cite{an2011refinement, sinha2018stackelberg, an2017stackelberg, blum2019computing, conitzer2006computing, gan2018stackelberg}.

\begin{table}
\renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{|c|c|c|}
    \hline Assumptions & Authors & Iteration Complexity \\
    \hline
    \multicolumn{3}{|c|}{Bilevel Optimization}\\
    \hline \hline 
    $\outerset = \R^\outerdim$, $\innerset = \R^\innerdim$, $\obj$ concave, $\otherobj$ strongly concave in $\inner$ & \citeauthor{ghadimi2018approximation} (\citeyear{ghadimi2018approximation}) & $\tilde{O}(\nicefrac{\kappa^3}{\varepsilon^2})$ \\
    \hline
    $\innerset = \R^\innerdim$, $\obj$ concave, $\otherobj$ strongly concave in $\inner$ & \citeauthor{ji2021bilevel} (\citeyear{ji2021bilevel}) & $\tilde{O}(\nicefrac{\kappa^4}{\varepsilon^2})$ \\
    \hline
    \hline
    \multicolumn{3}{|c|}{Bilevel optimization with multiobjective lower-level problem}\\
    \hline
    \hline
\end{tabular}
    \caption{Comparison of the best known computational complexities for bilevel optimization problems.}
    \label{tab:my_label}
\end{table}


\paragraph{Bilevel Multiobjective Optimization.}
A limited number of papers \cite{sinha2015multi, deb2009multi, ji2018multiobjective} have analyzed bilevel multiobjective optimization problems in which the upper- and lower-level problems \emph{both\/} have multiple objectives, i.e., Stackelberg games with multiple leaders and multiple followers.
These works focus on Stackelberg equilibria in which the leaders first, and the followers second, each play a Pareto-optimal solution, and do not provide polynomial-time computation guarantees. 

There also exists a parallel line of work within game theory on computing Stackelberg-Nash equilibrium in Stackelberg-Nash games \cite{nakamura2015one, liu1998stackelberg}.
These papers provide convergence guarantees to various notions of first-order Stackelberg-Nash equilibria, as it is not possible to compute a Stackelberg-Nash equilibrium in polynomial-time in the games the authors consider \cite{basilico2020bilevel, coniglio2020computing}.
A more recent line of work provides a first-order method to compute a Stackelberg-Nash equilibrium when the followers are assumed \samy{}{(by fiat)} \amy{i want that this assumption is totally unrealistic!} to play a unique Nash equilibrium, by using variants of the implicit function theorem and the envelope theorem \cite{li2020end, li2022solving, sinha2019using, wang2022coordinating}.

A more recent line of work has turned its attention to multiple leader-multiple follower Stackelberg games.
These works have once again focused on computing stationary solution concepts rather than Nash-Stackelberg-Nash equilibria, \amy{did you make up this name? or did Solis or Sinha?}\deni{These guys did not make it up but other people did. see \url{https://arxiv.org/abs/2202.11880}} i.e., Stackelberg equilibria at which the leaders play a Nash assuming the followers play a Nash \cite{solis2016modeling, sinha2014finding}. 
Finally, \citeauthor{gu2023min} (\citeyear{gu2023min}) provide polynomial-time computational guarantees for robust solutions to %multiobjective bilevel optimization problems with multiple leaders and multiple followers,
Nash-Stackelberg-Nash games, which can be seen as variants of weak Nash-Stackelberg-Nash equilibrium, under the assumption that the followers' payoffs are strongly convex.


\paragraph{Computation of competitive equilibrium}
The study of the computational complexity of competitive equilibria was initiated by \citet{devanur2002market}, who provided a polynomial-time method for computing competitive equilibrium in a special case of the Arrow-Debreu (exchange) market model, namely Fisher markets, when buyers utilities are linear.
\citet{jain2005market} subsequently showed that a large class of Fisher markets with homogeneous utility functions could be solved in polynomial-time using interior point methods.
Recently, \citet{gao2020polygm} studied an alternative family of first-order methods for solving Fisher markets, assuming linear, quasilinear, and Leontief utilities, as such methods can be more efficient when markets are large.

Devising algorithms for the computation of competitive equilibrium in general Arrow-Debreu markets is still an active area of research.
While the computation of competitive equilibrium is PPAD-complete in general, \amy{i cannot parse the rest of this sentence. it's a run-on, for sure!} Arrow-Debreu markets with additively separable, piecewise-linear and concave utilities \cite{chen2006settling}, and the computation of competitive equilibrium in Arrow-Debreu markets with Leontief buyers being equivalent to the computation of Nash equilibrium in bimatrix games \cite{codenotti2006leontief, deng2008computation}, there exists polynomial-time algorithms to compute competitive equilibrium for special cases of Arrow-Debreu markets, including markets whose excess demand satisfies the weak gross substitutes (WGS) condition \cite{codenotti2005market, bei2015tatonnement}, Arrow-Debreu markets with buyers whose utilities are linear \cite{garg2004auction, branzei2021proportional} or CES utilities in the weak gross substitutes range \cite{branzei2021proportional}.


==> static_fisher_market.tex <==
\subsubsection{Static Fisher Markets\sadie{one-shot?}}

A \mydef{(one-shot) Fisher market} $\calM \doteq (\numbuyers, \numgoods, \util, \type, \budget)$ consists of $\numbuyers$ buyers and $\numgoods$ divisible goods with unit supply\citep{brainard2000compute}. The set of \mydef{Competitive Equilibrium (CE)} of any Fisher market $(\numbuyers, \numgoods, \util, \type, \budget)$ with continuous, concave, and homogeneous\footnote{A function $f: \R^m \to \R$ is called \mydef{homogeneous of degree $k$} if $\forall \allocation[ ] \in \R^m, \lambda > 0, f(\lambda \allocation[ ]) = \lambda^k f(\allocation[ ])$.} utility functions is equal to the set of Nash equilibria of the \mydef{Eisenberg-Gale min-max game} (defined in \Cref{eq:eg_game}),%
\footnote{This min-max game corresponds to the Lagrangian saddle-point formulation of the Eisenberg-Gale program \cite{gale1989theory, jain2005market}.} 
a convex-concave min-max game between a seller who chooses prices $\price \in \R_+^{\numgoods}$ and buyers who collectively choose allocations
$\allocation \in \R_+^{\numbuyers \times \numgoods}$ (more details see \Cref{sec_app:markets}).


Therefore, for any Fisher market $\calM \doteq (\numbuyers, \numgoods, \util, \typetrue, \budgettrue)$, 
we can construct a inverse game $\game[][-1] \doteq 
(\game[][\paramtrue]/\paramtrue , \truestrat)$ where $\game[][\paramtrue]$ is the corresponding Eisenberg-Gale min-max game (\Cref{eq:eg_game}) parameterized by the true types and budgets $\paramtrue=(\typetrue, \budgettrue)$, and $\truestrat=(\allocation[][][][*], \price^*)$ is not only a NE of the game $\game[][\paramtrue]$ but also a CE of market $\calM$. Our goal is to recover the true market parameters $\paramtrue=(\typetrue, \budgettrue)$ given the observed $\truestrat=(\allocation[][][][*], \price^*)$, by solving this inverse game problem using \Cref{thm:inverse_NE} and \Cref{alg:gda}. 



We ran two different experiments\footnote{We include a detailed description of our experimental setup in the appendix.}. First, we solved a simpler inverse game problem where the true type $\typetrue$ is given, and we just need to retrieve the true budgets $\budgettrue$; then, we attempt to recover both true type and true budgets simultaneously. For both experiments, we created 500 markets with each of these three (standard) classes of utility functions parameterized by types:
1.~\mydef{linear}: $\util[\buyer](\allocation[\buyer]; \type[\buyer]) = \sum_{\good \in \goods} \type[\buyer][\good] \allocation[\buyer][\good]$; 2.~\mydef{Cobb-Douglas (CD)}:  $\util[\buyer](\allocation[\buyer]; \type[\buyer]) = \prod_{\good \in \goods} {\allocation[\buyer][\good]}^{\type[\buyer][\good]}$; and 3.~\mydef{Leontief}:  $\util[\buyer](\allocation[\buyer]; \type[\buyer]) = \min_{\good \in \goods} \left\{ \frac{\allocation[\buyer][\good]}{\type[\buyer][\good]}\right\}$. 
Then, we ran \Cref{alg:gda} on min-max optimization problem \sadie{I may write out the specific min-max problem for fisher, but I don't think we have enough space. Maybe in the Appendix.} defined in \Cref{eq:min_max_gen_sim} to compute the inverse Nash Equilibrium of the inverse game $\game[][-1]$ defined above.
Finally, for each utility type, we recorded the percentage of markets that we could recover the true parameters, i.e., the markets for which our computed parameters is close enough to the true parameters, and the average exploitability\sadie{refer appendix?} of the observed equilibrium evaluated under the computed parameters across all markets.
% To compute the true budgets, we solve the min-max optimization problem \begin{align}\label{eq:fisher_min_max_budgets}
%         \min_{\substack{\budget \in \R_+^{\numbuyers}}} \max_{\substack{\allocation\in \R_+^{\numbuyers\times\numgoods\\
%         \price\in \R_+^{\numgoods}  }}}
%         \underbrace{
%         \left( -\obj(\price, \allocation[][][][*]; \typetrue, \budget)+ \obj(\price^*, \allocation[][][][*]; \typetrue, \budget)
%         \right) + \left(\obj(\price^*, \allocation; \typetrue, \budget)- \obj(\price^*, \allocation[][][][*]; \typetrue, \budget)\right)
%         }_{ = \cumulregret[] ((\allocation[][][][*], \price^*), (\allocation,\price); \budget)}
% \end{align}
% using \Cref{alg:gda}.

\Cref{table:fisher_results} shows that when only retrieving budgets,we were able to recover all the parameters and minimize exploitability in markets with Linear and Cobb-Douglas utilities, but we hardly do so in Leontief markets. The difficulty in this case likely arises from two aspects: first, Leontief utility function is not differentiable, so the min-max optimization problems associated to Leontief
markets are not smooth; moreover, for any Leontief Fisher market, the CE is not guaranteed to be unique. 
When computing budgets and types at once, while our algorithm can still minimize exploitability for both Linear nad Cobb-Douglas markets, it cannot really retrive true parameters in Linear markets. This may due to the fact that, in Linear markets, though competitive equilibrium prices are unique, the competitive allocations are not guaranteed to be unique; by contrast, the CEs are always unique in Leontief markets. 

==> stoch_fisher_market.tex <==
\subsubsection{Stochastic Fisher Markets}

% A \mydef{(one-shot) Fisher market} consists of $\numbuyers$ buyers and $\numgoods$ divisible goods \citep{brainard2000compute}.
% Each buyer $\buyer \in \buyers$ is endowed with a budget $\budget[\buyer] \in \budgetspace[\buyer] \subseteq \mathbb{R}_{+}$ and a utility function $\util[\buyer]: \mathbb{R}_{+}^{\numgoods} \times \typespace[\buyer] \to \mathbb{R}$, which is parameterized by a type $\type[\buyer] \in \typespace[\buyer]$ that defines a preference relation over the consumption space $\R^\numgoods_+$.
% % \amy{you should introduce types here, if it is types that define utility functions!}
% % \footnote{\sdeni{WLOG, we assume that all budgets are strictly positive; otherwise, we could remove a buyer with a zero budget without affecting the equilibrium.}{}} 
% %As is standard in the literature, we assume that there is one divisible unit of each good in the market.
% Each good is characterized by a supply $\supply[\good] \in \supplyspace[\good] \subset \R_+$.


% An instance of a Fisher market is then a tuple $\calM \doteq (\numbuyers, \numgoods, \util, \type, \budget, \supply)$, where $\util \doteq \left(\util[1], \hdots, \util[\numbuyers] \right)$ is a vector-valued function of all utility functions,
% %\amy{why do you need utility functions in this market spec if you have types?}\deni{Type for me is the valuations that parameterize for instance linear utilities, utility functions are the actual form, i.e., they \amy{the utility functions?} describe whether if we have linear, CD, or Leontief utilities, then the type describes the utility function's parameters.} \sadie{I think in the static Fisher market model, we assumed that different buyers may have different class (linear, leontief, cd, or so) of utility, while type gives the specific valuations. That is, $u_i\in \{linear, leontief, cd\}$, while $t_i$ is some array of coefficients? But I thought the name ``type" is a little misleading, and maybe ``valuation" or ``coefficient" is more straight forward?}
% $\budget \doteq (\budget[1], \hdots, \budget[\numbuyers]) \in \R_{+}^{\numbuyers}$ is the vector of buyer budgets, and $\supply \doteq (\supply[1], \hdots, \supply[\numgoods]) \in \R_{+}^{\numgoods}$ is the vector of supplies.
% When clear from context, we simply denote $\calM$
% %$(\numbuyers, \numgoods, \util, \type, \budget, \supply)$ 
% by $(\type, \budget, \supply)$.

% Given a Fisher market $(\type, \budget, \supply)$, an \mydef{allocation} $\allocation = \left(\allocation[1], \hdots, \allocation[\numbuyers] \right)^T \in \R_+^{\numbuyers \times \numgoods}$ is a map from goods to buyers, represented as a matrix, s.t. $\allocation[\buyer][\good] \ge 0$ denotes the amount of good $\good \in \goods$ allocated to buyer $\buyer \in \buyers$. Goods are assigned \mydef{prices} $\price = \left(\price[1], \hdots, \price[\numgoods] \right)^T \in \mathbb{R}_+^{\numgoods}$. A tuple $(\allocation[][][][*], \price^*)$ is said to be a \mydef{competitive equilibrium (CE)} \citep{arrow-debreu, walras} if 
% 1.~buyers are utility maximizing, constrained by their budget, i.e., $\forall \buyer \in \buyers, \allocation[\buyer][][][*] \in \argmax_{\allocation[ ] : \allocation[ ] \cdot \price^* \leq \budget[\buyer]} \util[\buyer](\allocation[ ], \type[\buyer])$;
% and 2.~the market clears, i.e., $\forall \good \in \goods,  \price[\good]^* > 0 \Rightarrow \sum_{\buyer \in \buyers} \allocation[\buyer][\good][][*] = \supply[\good]$ and $\price[\good]^* = 0 \Rightarrow\sum_{\buyer \in \buyers} \allocation[\buyer][\good][][*] \leq \supply[\good]$.

% \amy{move to appendix!}
%\samy{We denote the type space of all buyers $\typespace = \bigtimes_{\buyer \in \buyers} \typespace[\buyer]$, and the space of all possible budgets for all buyers $\budgetspace = \bigtimes_{\buyer \in \buyers} \budgetspace[\buyer]$. We denote the set of all goods' possible supplies $\supplyspace = \bigtimes_{\good \in \goods} \supplyspace[\good]$.}{}\deni{This should not be removed, it is used in the appendix, and is also our state space, it's important!}\amy{if it is not used in the main body, just define it in the appendix. if you want to use it here, it goes above the previous paragraph so you can then say $(t,b,q) \in T \times B \times Q$.}


A \mydef{stochastic Fisher market with savings} $\fishermkt[0] \doteq (\numbuyers, \numgoods, \util, \states, \initstates, \trans, \discount)$ is a repeated market that travels through a sequence of states in which each state corresponds to a (one-shot) Fisher market (more details see \Cref{sec_app:markets}).
The market is initialized at state $\staterv[0] \sim \initstates$, and for each state $\staterv[\iter] \in \states$ encountered at time step $\iter \in \N_+$, the market determines the prices $\price[][\iter]$ of the goods, while the buyers choose their allocations $\allocation[][][\iter]$ and set aside some \mydef{savings} $\saving[\buyer][\iter] \in [0, \budget[\buyer]]$ to potentially spend at some future state.
Once allocations, savings, and prices have been determined, the market terminates with probability $1-\discount$, or it transitions to a new state $\staterv[\iter + 1] = \state^\prime$ with probability $\discount \trans(\state^\prime \mid \state, \saving)$, depending on the buyers' saving decisions.%
We denote a stochastic Fisher market by $\fishermkt[0] \doteq (\numbuyers, \numgoods, \util, \states, \initstates, \trans, \discount)$.

Given a stochastic Fisher market with savings $\fishermkt[0]$
%$(\states, \util, \state[0], \trans, \discount)$, 
a \mydef{recursive competitive equilibrium (recCE)} \citep{mehra1977recursive} is a tuple $(\allocation[][][][*], \saving[][][*], \price^*) \in \R_+^{\numbuyers \times \numgoods \times \states} \times \R_+^{\numbuyers \times \states} \times \R_+^{\numgoods \times \states}$, which consists of stationary \mydef{allocation}, \mydef{savings}, and \mydef{pricing policies} s.t.\ 1) the buyers are expected utility maximizers, constrained by their savings and spending constraints, i.e., for all buyers $\buyer \in \buyers$, $(\allocation[\buyer][][][*], \saving[\buyer][][*])$ is an optimal policy that, for all states $\state \doteq (\type, \budget, \supply) \in \states$, solves the \mydef{consumption-savings problem}, defined by the following Bellman equations: for all $\state \in \states$
\begin{align}
    \budgetval[\buyer](\state) = \max_{(\allocation[\buyer], \saving[\buyer]) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot \price^*(\state) + \saving[\buyer] \leq \budget[\buyer]} \left\{ \util[\buyer]\left(\allocation[\buyer], \type[\buyer]\right)     + \discount \Ex_{({\type}^\prime, {\budget}^\prime, {\supply}^\prime) \sim \trans(\cdot \mid \state, (\allocation[\buyer], \allocation[][][][*]_{-\buyer}(\state)), 
    (\saving[\buyer], \saving[][][*]_{-\buyer}(\state)))} 
    \left[ \budgetval[\buyer]({\type}^\prime, {\budget}^\prime + (\saving[\buyer], \saving[][][*]_{-\buyer}(\state)), {\supply}^\prime) \right]  \right\},    
\end{align}
    %\budgetval[\buyer](\type, \budget, \supply) =
    

%for all states $(\type, \budget, \supply) \in \states$ 
where $\allocation[][][][*]_{-\buyer}$, $\saving[][][*]_{-\buyer}$ denote the 
%competitive equilibrium 
allocation and saving policies excluding buyer $\buyer$; and
2) the market clears in each state so that unallocated goods in each state are priced at 0, i.e., for all $\good \in \goods$ and $\state \in \states$,
$    
        \price[\good]^*(\state) > 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good][][*](\state) = \supply[\good]
$ and
$
        \price[\good]^*(\state) \geq 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good][][*](\state) \leq \supply[\good]
$.
% \samy{By analogy with Markov perfect equilibrium, we can view a}
A recCE is Markov perfect, as it is a CE regardless of initial  state,%
\footnote{Just as any stochastic game can be (non-compactly) represented as a one-shot game, any stochastic Fisher market with savings can be represented as a one-shot Fisher market comprising the same buyers (with utility functions given by their discounted cumulative expected utility) 
% $\Ex_{\staterv[\iter]} \left[\discount^\iter \util[\buyer]\left(\allocation[\buyer][][\iter], \type[\buyer][][\iter]\right) \right]$
and the same goods, enhanced with time-stamps.
It has been shown that competitive equilibria exist in such markets~\citep{prescott1972note}.
In particular, a recCE is a CE in this market; the time stamps ensure that the market clears at every time step, as required.}
%\amy{does whoever writes about the time-stamped construction prove that CE exist in these one-shot markets? also, would a recursive CE of the stochastic Fisher market also be a CE of this one-shot market?}
i.e., buyers are allocated expected discounted cumulative utility-maximizing goods regardless of initial state, and the aggregate demand for each good is equal to its aggregate supply \emph{at all states}.

We show that the computation of a recursive competitive equilibrium in stochastic Fisher markets is equivalent to the computation of nash equilibrium in zero-sum Markov game
